A Benchmark of JSON-compatible Binary Serialization Specifications

We present a comprehensive benchmark of JSON-compatible binary serialization specifications using the SchemaStore open-source test suite collection of over 400 JSON documents matching their respective schemas and representative of their use across industries. We benchmark a set of schema-driven (ASN.1, Apache Avro, Microsoft Bond, Cap'n Proto, FlatBuffers, Protocol Buffers, and Apache Thrift) and schema-less (BSON, CBOR, FlexBuffers, MessagePack, Smile, and UBJSON) JSON-compatible binary serialization specifications. Existing literature on benchmarking JSON-compatible binary serialization specifications demonstrates extensive gaps when it comes to binary serialization specifications coverage, reproducibility and representativity, the role of data compression in binary serialization and the choice and use of obsolete versions of binary serialization specifications. We introduce a tiered taxonomy for JSON documents consisting of 36 categories classified as Tier 1, Tier 2 and Tier 3 as a common basis to class JSON documents based on their size, type of content, characteristics of their structure and redundancy criteria. We built and published a free-to-use online tool to automatically categorize JSON documents according to our taxonomy that generates related summary statistics. In the interest of fairness and transparency, we adhere to reproducible software development standards and publicly host the benchmark software and results on GitHub.

==> boxplots/circleciblank.tex <==
In \autoref{fig:benchmark-circleciblank-boxplot}, we observe the medians for
uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications. The
range between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications is smaller than
the range between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications. However, their
respective quartiles overlap.

% Compression

In terms of compression, GZIP results in the lower median for schema-driven
binary serialization specifications while LZ4 results in the lower median for
schema-less binary serialization specifications. However, compression is not
space-efficient in terms of the median for both schema-driven and schema-less
binary serialization specifications. Additionally, the use of GZIP and LZMA for
schema-driven binary serialization specifications exhibit upper outliers. While
compression does not contribute to space-efficiency, it reduces the range
between the upper and lower whiskers and inter-quartile range for schema-driven
binary serialization specifications and it reduces the inter-quartile range for
schema-less binary serialization specifications.  In particular, the
compression format with the smaller range between the upper and lower whiskers
for schema-driven binary serialization specifications is GZIP, the compression
formats with the smaller inter-quartile range for schema-driven binary
serialization specifications are GZIP and LZMA, and the compression format with
the smaller inter-quartile range for schema-less binary serialization
specifications is LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less
binary serialization specifications and that compression does not contribute to
space-efficiency in comparison to both uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/circlecimatrix.tex <==
In \autoref{fig:benchmark-circlecimatrix-boxplot}, we observe the medians for
uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications is smaller than the
range between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications.

% Compression

In terms of compression, LZMA results in the lower median for schema-driven
binary serialization specifications while GZIP results in the lower median for
schema-less binary serialization specifications. However, compression is not
space-efficient in terms of the median for both schema-driven and schema-less
binary serialization specifications. Additionally, the use of GZIP, LZ4 and
LZMA for schema-driven binary serialization specifications exhibit upper
outliers.  While compression does not contribute to space-efficiency, it
reduces the range between the upper and lower whiskers and inter-quartile range
for both schema-driven and schema-less binary serialization specifications.  In
particular, the compression format with the smaller range between the upper and
lower whiskers and the smaller inter-quartile range for schema-driven binary
serialization specifications is LZMA, the compression formats with the smaller
range between the upper and lower whiskers for schema-less binary serialization
specifications are GZIP and LZMA, and the compression format with the smaller
inter-quartile range for schema-less binary serialization specifications is
LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less binary
serialization specifications and that compression does not contribute to
space-efficiency in comparison to both uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/commitlint.tex <==
In \autoref{fig:benchmark-commitlint-boxplot}, we observe the medians for
uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications is smaller than the range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications. However, their
respective quartiles overlap.

% Compression

In terms of compression, GZIP results in the lower median for both
schema-driven and schema-less binary serialization specifications.
Additionally, GZIP and LZMA are space-efficient in terms of the median in
comparison to uncompressed schema-driven binary serialization specifications
and GZIP, LZ4 and LZMA are space-efficient in terms of the median in comparison
to uncompressed schema-less binary serialization specifications. However, the
use of GZIP and LZ4 for schema-driven binary serialization specifications
exhibit upper outliers.  Nevertheless, compression reduces the range between
the upper and lower whiskers and inter-quartile range for schema-driven binary
serialization specifications.  In particular, the compression format with the
smaller range between the upper and lower whiskers for schema-driven binary
serialization specifications is GZIP, the compression format with the smaller
inter-quartile range for schema-driven binary serialization specifications is
LZMA, and the compression formats with the smaller range between the upper and
lower whiskers and the smaller inter-quartile range for schema-less binary
serialization specifications are GZIP and LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less
binary serialization specifications. GZIP and LZMA are space-efficient in
comparison to uncompressed schema-driven binary serialization specifications
and all the considered compression formats are space-efficient in comparison to
uncompressed schema-less binary serialization specifications.


==> boxplots/commitlintbasic.tex <==
In \autoref{fig:benchmark-commitlintbasic-boxplot}, we observe the medians for
uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications is smaller than the range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications.

% Compression

In terms of compression, LZ4 results in the lower median for both schema-driven
and schema-less binary serialization specifications.  However, compression is
not space-efficient in terms of the median for both schema-driven and
schema-less binary serialization specifications.  While compression does not
contribute to space-efficiency, it reduces the range between the upper and
lower whiskers and inter-quartile range for schema-driven binary serialization
specifications.  In particular, the compression formats with the smaller range
between the upper and lower whiskers for schema-driven binary serialization
specifications are GZIP and LZMA, the compression format with the smaller
inter-quartile range for schema-driven binary serialization specifications is
LZMA, and the compression format with the smaller inter-quartile range for
schema-less binary serialization specifications is GZIP.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less binary
serialization specifications and that compression does not contribute to
space-efficiency in comparison to both uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/epr.tex <==
In \autoref{fig:benchmark-epr-boxplot}, we observe the medians for uncompressed
schema-driven binary serialization specifications to be smaller in comparison to
uncompressed schema-less binary serialization specifications.  The range between the
upper and lower whiskers and the inter-quartile range of uncompressed
schema-less binary serialization specifications is smaller than the range between the
upper and lower whiskers and the inter-quartile range of uncompressed
schema-driven binary serialization specifications.

% Compression

In terms of compression, LZMA results in the lower median for both
schema-driven and schema-less binary serialization specifications.
Additionally, GZIP, LZ4 and LZMA are space-efficient in terms of the median in
comparison to both uncompressed schema-driven and schema-less binary
serialization specifications.  However, the use of GZIP for schema-less binary
serialization specifications exhibit upper outliers.  Nevertheless, compression
reduces the range between the upper and lower whiskers and inter-quartile range
for both schema-driven and schema-less binary serialization specifications.  In
particular, the compression format with the smaller range between the upper and
lower whiskers and the smaller inter-quartile range for schema-driven binary
serialization specifications is LZMA, the compression format with the smaller
range between the upper and lower whiskers for schema-less binary serialization
specifications is GZIP, and the compression formats with the smaller
inter-quartile range for schema-less binary serialization specifications are
GZIP and LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less
binary serialization specifications and that all the considered compression
formats are space-efficient in comparison to uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/eslintrc.tex <==
In \autoref{fig:benchmark-eslintrc-boxplot}, we observe the medians for
uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications is smaller than the
range between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications.

% Compression

In terms of compression, LZMA results in the lower median for schema-driven
binary serialization specifications while GZIP results in the lower median for
schema-less binary serialization specifications.  Additionally, GZIP and LZMA are
space-efficient in terms of the median in comparison to uncompressed
schema-driven binary serialization specifications and GZIP, LZ4 and LZMA are
space-efficient in terms of the median in comparison to uncompressed
schema-less binary serialization specifications.  However, the use of LZ4 for
schema-driven binary serialization specifications and the use of GZIP, LZ4 and LZMA
for schema-less binary serialization specifications exhibit upper outliers.
Nevertheless, compression reduces the range between the upper and lower
whiskers and inter-quartile range for both schema-driven and schema-less binary
serialization specifications.  In particular, the compression format with the smaller
range between the upper and lower whiskers for schema-driven binary
serialization specifications is LZ4, and the compression format with the smaller range
between the upper and lower whiskers and the smaller inter-quartile range for
schema-less binary serialization specifications is LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less binary
serialization specifications. GZIP and LZMA are space-efficient in comparison to
uncompressed schema-driven binary serialization specifications and all the considered
compression formats are space-efficient in comparison to uncompressed
schema-less binary serialization specifications.


==> boxplots/esmrc.tex <==
In \autoref{fig:benchmark-esmrc-boxplot}, we observe the medians for
uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications is smaller than the range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications.

% Compression

In terms of compression, LZ4 results in the lower median for schema-driven
binary serialization specifications while GZIP results in the lower median for
schema-less binary serialization specifications.  However, compression is not
space-efficient in terms of the median for both schema-driven and schema-less
binary serialization specifications.  Additionally, the use of LZ4 for
schema-driven binary serialization specifications exhibits upper outliers.
While compression does not contribute to space-efficiency, it reduces the range
between the upper and lower whiskers and inter-quartile range for both
schema-driven and schema-less binary serialization specifications.  In
particular, the compression format with the smaller range between the upper and
lower whiskers and the smaller inter-quartile range for schema-driven binary
serialization specifications is LZMA, the compression format with the smaller
range between the upper and lower whiskers for schema-less binary serialization
specifications is GZIP, and the compression formats with the smaller
inter-quartile range for schema-less binary serialization specifications are
GZIP and LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less binary
serialization specifications and that compression does not contribute to
space-efficiency in comparison to both uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/geojson.tex <==
In \autoref{fig:benchmark-geojson-boxplot}, contrary to other cases, we observe
the medians for uncompressed schema-less binary serialization specifications to be
smaller in comparison to uncompressed schema-driven binary serialization
specifications.  The range between the upper and lower whiskers of uncompressed
schema-less binary serialization specifications is smaller than the range between the
upper and lower whiskers of uncompressed schema-driven binary serialization
specifications.  However, the inter-quartile range of uncompressed schema-less binary
serialization specifications is larger than the inter-quartile range of uncompressed
schema-driven binary serialization specifications. Additionally, their respective
quartiles overlap.

% Compression

In terms of compression, LZMA results in the lower median for both
schema-driven and schema-less binary serialization specifications.
Additionally, GZIP, LZ4 and LZMA are space-efficient in terms of the median in
comparison to both uncompressed schema-driven and schema-less binary
serialization specifications.  However, the use of GZIP, LZ4 and LZMA for
schema-driven binary serialization specifications exhibits upper outliers.
Nevertheless, compression reduces the range between the upper and lower
whiskers and inter-quartile range for both schema-driven and schema-less binary
serialization specifications.  In particular, the compression formats with the
smaller range between the upper and lower whiskers and the smaller
inter-quartile range for schema-driven binary serialization specifications are
GZIP and LZMA, the compression format with the smaller range between the upper
and lower whiskers for schema-less binary serialization specifications is LZMA,
and the compression formats with the smaller inter-quartile range for
schema-less binary serialization specifications are GZIP and LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-less binary serialization
specifications are space-efficient in comparison to uncompressed schema-driven
binary serialization specifications and that all the considered compression
formats are space-efficient in comparison to uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/githubfundingblank.tex <==
In \autoref{fig:benchmark-githubfundingblank-boxplot}, we observe the medians
for uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications is smaller than the range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications.

% Compression

In terms of compression, LZ4 results in the lower median for schema-driven
binary serialization specifications while GZIP results in the lower median for
schema-less binary serialization specifications.  Compression is not
space-efficient in terms of the median in comparison to uncompressed
schema-driven binary serialization specifications. However, GZIP is
space-efficient in terms of the median in comparison to uncompressed
schema-less binary serialization specifications.  Nevertheless, compression
reduces the range between the upper and lower whiskers and inter-quartile range
for both schema-driven and schema-less binary serialization specifications.  In
particular, the compression format with the smaller range between the upper and
lower whiskers and the smaller inter-quartile range for both schema-driven and
schema-less binary serialization specifications is LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less binary
serialization specifications. Compression does not contribute to space-efficiency in
comparison to schema-driven binary serialization specifications but GZIP is
space-efficient in comparison to schema-less binary serialization specifications.


==> boxplots/githubworkflow.tex <==
In \autoref{fig:benchmark-githubworkflow-boxplot}, we observe the medians for
uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications is smaller than the range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications. However, their
respective quartiles overlap.

% Compression

In terms of compression, GZIP and LZMA result in the lower medians for
schema-driven binary serialization specifications while GZIP results in the
lower median for schema-less binary serialization specifications.
Additionally, GZIP and LZMA are space-efficient in terms of the median in
comparison to uncompressed schema-driven binary serialization specifications
and GZIP, LZ4 and LZMA are space-efficient in terms of the median in comparison
to uncompressed schema-less binary serialization specifications.  Also,
compression reduces the range between the upper and lower whiskers and
inter-quartile range for both schema-driven and schema-less binary
serialization specifications.  In particular, the compression format with the
smaller range between the upper and lower whiskers and the smaller
inter-quartile range for schema-driven binary serialization specifications is
LZMA, the compression formats with the smaller range between the upper and
lower whiskers for schema-less binary serialization specifications are GZIP and
LZMA, and the compression format with the smaller inter-quartile range for
schema-less binary serialization specifications is GZIP.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less
binary serialization specifications. GZIP and LZMA are space-efficient in
comparison to uncompressed schema-driven binary serialization specifications
and all the considered compression formats are space-efficient in comparison to
uncompressed schema-less binary serialization specifications.


==> boxplots/gruntcontribclean.tex <==
In \autoref{fig:benchmark-gruntcontribclean-boxplot}, we observe the medians
for uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications is smaller than the range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications.

% Compression

In terms of compression, GZIP results in the lower median for both
schema-driven and schema-less binary serialization specifications.  However,
compression is not space-efficient in terms of the median for both
schema-driven and schema-less binary serialization specifications.  While
compression does not contribute to space-efficiency, it reduces the range
between the upper and lower whiskers and inter-quartile range for both
schema-driven and schema-less binary serialization specifications.  In
particular, the compression format with the smaller range between the upper and
lower whiskers for schema-driven binary serialization specifications is LZMA,
the compression formats with the smaller inter-quartile range for schema-driven
binary serialization specifications are GZIP and LZMA, the compression formats
with the smaller range between the upper and lower whiskers for schema-less
binary serialization specifications are GZIP and LZ4, and the compression
formats with the smaller inter-quartile range for schema-less binary
serialization specifications are GZIP and LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less binary
serialization specifications and that compression does not contribute to
space-efficiency in comparison to both uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/imageoptimizerwebjob.tex <==
In \autoref{fig:benchmark-imageoptimizerwebjob-boxplot}, we observe the medians
for uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications is smaller than the range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications.

% Compression

In terms of compression, LZ4 results in the lower median for schema-driven
binary serialization specifications while GZIP results in the lower median for
schema-less binary serialization specifications.  However, compression is not
space-efficient in terms of the median for both schema-driven and schema-less
binary serialization specifications.  While compression does not contribute to
space-efficiency, it reduces the range between the upper and lower whiskers and
inter-quartile range for both schema-driven and schema-less binary
serialization specifications.  In particular, the compression format with the
smaller range between the upper and lower whiskers for schema-driven binary
serialization specifications is LZMA, the compression formats with the smaller
inter-quartile range for schema-driven binary serialization specifications are
GZIP and LZMA, the compression format with the smaller range between the upper
and lower whiskers for schema-less binary serialization specifications is GZIP,
and the compression format with the smaller inter-quartile range for
schema-less binary serialization specifications is LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less binary
serialization specifications and that compression does not contribute to
space-efficiency in comparison to both uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/jsonereversesort.tex <==
In \autoref{fig:benchmark-jsonereversesort-boxplot}, we observe the medians for
uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications is smaller than the range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications. However, their
respective quartiles overlap.

% Compression

In terms of compression, GZIP, LZ4 and LZMA resuls in similar medians for
schema-driven binary serialization specifications while GZIP results in the
lower median for schema-less binary serialization specifications.  However,
compression is not space-efficient in terms of the median for both
schema-driven and schema-less binary serialization specifications.
Additionally, the use of LZ4 for schema-driven binary serialization
specifications exhibits upper outliers.  While compression does not contribute
to space-efficiency, it reduces the range between the upper and lower whiskers
and inter-quartile range for both schema-driven and schema-less binary
serialization specifications.  In particular, the compression formats with the
smaller range between the upper and lower whiskers for schema-driven binary
serialization specifications are GZIP and LZMA, the compression formats with
the smaller inter-quartile range for schema-driven binary serialization
specifications are GZIP and LZMA, the compression formats with the smaller
range between the upper and lower whiskers for schema-less binary serialization
specifications are GZIP and LZMA, and the compression format with the smaller
inter-quartile range for schema-less binary serialization specifications is
LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less binary
serialization specifications and that compression does not contribute to
space-efficiency in comparison to both uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/jsonesort.tex <==
In \autoref{fig:benchmark-jsonesort-boxplot}, we observe the medians for
uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers of uncompressed schema-less binary
serialization specifications is smaller than the range between the upper and lower
whiskers of uncompressed schema-driven binary serialization specifications.  However,
the inter-quartile range of both both uncompressed schema-driven and
schema-less binary serialization specifications is similar.  Additionally, their
respective quartiles overlap.

% Compression

In terms of compression, GZIP and LZ4 result in the lower medians for
schema-driven binary serialization specifications while LZ4 results in the
lower median for schema-less binary serialization specifications.  However,
compression is not space-efficient in terms of the median for both
schema-driven and schema-less binary serialization specifications.
Additionally, the use of LZ4 for both schema-driven binary serialization
specifications and schema-less binary serialization specifications exhibits
upper outliers.  While compression does not contribute to space-efficiency, it
reduces the range between the upper and lower whiskers and inter-quartile range
for schema-driven binary serialization specifications and it reduces the
inter-quartile range for schema-less binary serialization specifications.  In
particular, the compression format with the smaller range between the upper and
lower whiskers for schema-driven binary serialization specifications is LZMA,
the compression formats with the smaller inter-quartile range for schema-driven
binary serialization specifications are GZIP and LZMA, the compression format
with the smaller range between the upper and lower whiskers for schema-less
binary serialization specifications is LZ4, and the compression formats with
the smaller inter-quartile range for schema-less binary serialization
specifications are GZIP and LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less
binary serialization specifications and that compression does not contribute to
space-efficiency in comparison to both uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/jsonfeed.tex <==
In \autoref{fig:benchmark-jsonfeed-boxplot}, we observe the medians for
uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications is smaller than the range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications.

% Compression

In terms of compression, GZIP and LZMA result in the lower medians for
schema-driven binary serialization specifications while GZIP results in the lower
median for schema-less binary serialization specifications.  Additionally, GZIP, LZ4
and LZMA are space-efficient in terms of the median in comparison to both
uncompressed schema-driven and schema-less binary serialization specifications.
However, the use of GZIP for schema-less binary serialization specifications exhibits
upper outliers.  Nevertheless, compression reduces the range between the upper
and lower whiskers and inter-quartile range for both schema-driven and
schema-less binary serialization specifications.  In particular, the compression
format with the smaller range between the upper and lower whiskers and the
smaller inter-quartile range for schema-driven binary serialization specifications is
LZMA, and the compression format with the smaller range between the upper and
lower whiskers and the smaller inter-quartile range for schema-less binary
serialization specifications is GZIP.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less
binary serialization specifications and that all the considered compression
formats are space-efficient in comparison to uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/jsonresume.tex <==
In \autoref{fig:benchmark-jsonresume-boxplot}, we observe the medians for
uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications is smaller than the range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications.

% Compression

In terms of compression, GZIP results in the lower median for both
schema-driven and schema-less binary serialization specifications.  Additionally,
GZIP, LZ4 and LZMA are space-efficient in terms of the median in comparison to
both uncompressed schema-driven and schema-less binary serialization specifications.
However, the use of LZMA for schema-less binary serialization specifications exhibits
upper outliers.  Nevertheless, compression reduces the range between the upper
and lower whiskers and inter-quartile range for both schema-driven and
schema-less binary serialization specifications.  In particular, the compression
format with the smaller range between the upper and lower whiskers and the
smaller inter-quartile range for both schema-driven and schema-less binary
serialization specifications is LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less
binary serialization specifications and that all the considered compression
formats are space-efficient in comparison to uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/netcoreproject.tex <==
In \autoref{fig:benchmark-netcoreproject-boxplot}, we observe the medians for
uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications is smaller than the range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications.

% compression

In terms of compression, LZMA results in the lower median for both
schema-driven and schema-less binary serialization specifications.
Additionally, GZIP, LZ4 and LZMA are space-efficient in terms of the median in
comparison to both uncompressed schema-driven and schema-less binary
serialization specifications.  However, the use of GZIP, LZ4 and LZMA for
schema-less binary serialization specifications exhibits upper outliers.
Nevertheless, compression reduces the range between the upper and lower
whiskers and inter-quartile range for both schema-driven and schema-less binary
serialization specifications.  In particular, the compression format with the
smaller range between the upper and lower whiskers for schema-driven binary
serialization specifications is LZMA, and the compression formats with the
smaller inter-quartile range for schema-driven binary serialization
specifications are GZIP and LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less
binary serialization specifications and that all the considered compression
formats are space-efficient in comparison to uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/nightwatch.tex <==
In \autoref{fig:benchmark-nightwatch-boxplot}, we observe the medians for
uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers of uncompressed schema-driven binary
serialization specifications is smaller than the range between the upper and lower
whiskers of uncompressed schema-less binary serialization specifications.  However,
the inter-quartile range of both both uncompressed schema-driven and
schema-less binary serialization specifications is similar.

% Compression

In terms of compression, GZIP and LZMA result in the lower medians for
schema-driven binary serialization specifications while GZIP results in the
lower median for schema-less binary serialization specifications.  Compression
is not space-efficient in terms of the median in comparison to uncompressed
schema-driven binary serialization specifications. However, GZIP, LZ4 and LZMA
are space-efficient in terms of the median in comparison to uncompressed
schema-less binary serialization specifications.  Additionally, the use of
GZIP, LZ4 and LZMA for both schema-driven binary serialization specifications
and schema-less binary serialization specifications exhibits upper outliers.
Nevertheless, compression reduces the range between the upper and lower
whiskers and inter-quartile range for both schema-driven and schema-less binary
serialization specifications.  In particular, the compression format with the
smaller inter-quartile range for schema-driven binary serialization
specifications is LZMA, the compression format with the smaller range between
the upper and lower whiskers for schema-less binary serialization
specifications is LZMA, and the compression format with the smaller
inter-quartile range for schema-less binary serialization specifications is
GZIP.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less binary
serialization specifications. Compression does not contribute to space-efficiency in
comparison to schema-driven binary serialization specifications but all the considered
compression formats are space-efficient in comparison to schema-less binary
serialization specifications.


==> boxplots/openweathermap.tex <==
In \autoref{fig:benchmark-openweathermap-boxplot}, we observe the medians for
uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers of uncompressed schema-driven and
schema-less binary serialization specifications is similar. However, the
inter-quartile range of uncompressed schema-driven binary serialization specifications
is smaller than the inter-quartile range of uncompressed schema-less binary
serialization specifications.

% Compression

In terms of compression, GZIP results in the lower medians for schema-driven
binary serialization specifications while LZMA results in the lower median for
schema-less binary serialization specifications.  Compression is not
space-efficient in terms of the median in comparison to uncompressed
schema-driven binary serialization specifications. However, GZIP and LZMA are
space-efficient in terms of the median in comparison to uncompressed
schema-less binary serialization specifications. Additionally, the use of GZIP,
LZ4 and LZMA for both schema-driven binary serialization specifications and
schema-less binary serialization specifications exhibits upper outliers.
Nevertheless, compression reduces the range between the upper and lower
whiskers and inter-quartile range for both schema-driven and schema-less binary
serialization specifications.  In particular, the compression format with the
smaller range between the upper and lower whiskers and the smaller
inter-quartile range for schema-driven binary serialization specifications is
LZMA, and the compression format with the smaller range between the upper and
lower whiskers and the smaller inter-quartile range for schema-less binary
serialization specifications is GZIP.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less binary
serialization specifications. Compression does not contribute to space-efficiency in
comparison to schema-driven binary serialization specifications but GZIP and LZMA are
space-efficient in comparison to uncompressed schema-less binary serialization
specifications.


==> boxplots/openweatherroadrisk.tex <==
In \autoref{fig:benchmark-openweatherroadrisk-boxplot}, we observe the medians
for uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications is smaller than the
range between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications.

% Compression

In terms of compression, GZIP results in the lower medians for schema-driven
binary serialization specifications while LZMA results in the lower median for
schema-less binary serialization specifications.  Additionally, GZIP and LZMA
are space-efficient in terms of the median in comparison to uncompressed
schema-driven binary serialization specifications and GZIP, LZ4 and LZMA are
space-efficient in terms of the median in comparison to uncompressed
schema-less binary serialization specifications.  However, the use of LZ4 for
schema-driven binary serialization specifications and the use of GZIP, LZ4 and
LZMA for schema-less binary serialization specifications exhibits upper
outliers.  Nevertheless, compression reduces the range between the upper and
lower whiskers and inter-quartile range for both schema-driven and schema-less
binary serialization specifications.  In particular, the compression format
with the smaller range between the upper and lower whiskers for schema-driven
binary serialization specifications is LZMA, the compression formats with the
smaller inter-quartile range for schema-driven binary serialization
specifications are GZIP and LZMA, and the compression format with the smaller
range between the upper and lower whiskers and the smaller inter-quartile range
for schema-less binary serialization specifications is GZIP.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less
binary serialization specifications. GZIP and LZMA are space-efficient in
comparison to uncompressed schema-driven binary serialization specifications
and all the considered compression formats are space-efficient in comparison to
uncompressed schema-less binary serialization specifications.


==> boxplots/packagejson.tex <==
In \autoref{fig:benchmark-packagejson-boxplot}, we observe the medians for
uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications is smaller than the range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications.

% Compression

In terms of compression, GZIP results in the lower median for both
schema-driven and schema-less binary serialization specifications.  Additionally,
GZIP, LZ4 and LZMA are space-efficient in terms of the median in comparison to
both uncompressed schema-driven and schema-less binary serialization specifications.
However, the use of GZIP and LZMA for schema-less binary serialization specifications
exhibits upper outliers.  Nevertheless, compression reduces the range between
the upper and lower whiskers and inter-quartile range for both schema-driven
and schema-less binary serialization specifications.  In particular, the compression
format with the smaller range between the upper and lower whiskers and the
smaller inter-quartile range for schema-driven binary serialization specifications is
LZMA, and the compression formats with the smaller range between the upper and
lower whiskers and the smaller inter-quartile range for schema-less binary
serialization specifications are GZIP and LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less
binary serialization specifications and that all the considered compression
formats are space-efficient in comparison to uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/packagejsonlintrc.tex <==
In \autoref{fig:benchmark-packagejsonlintrc-boxplot}, we observe the medians
for uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications is smaller than the range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications.

% Compression

In terms of compression, LZMA results in the lower medians for schema-driven
binary serialization specifications while GZIP and LZMA result in the lower
median for schema-less binary serialization specifications.  Additionally,
GZIP, LZ4 and LZMA are space-efficient in terms of the median in comparison to
both uncompressed schema-driven and schema-less binary serialization
specifications.  However, the use of GZIP, LZ4 and LZMA for schema-less binary
serialization specifications exhibits upper outliers.  Nevertheless,
compression reduces the range between the upper and lower whiskers and
inter-quartile range for both schema-driven and schema-less binary
serialization specifications.  In particular, the compression format with the
smaller range between the upper and lower whiskers and the smaller
inter-quartile range for schema-driven binary serialization specifications is
LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less
binary serialization specifications and that all the considered compression
formats are space-efficient in comparison to uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/sapcloudsdkpipeline.tex <==
In \autoref{fig:benchmark-sapcloudsdkpipeline-boxplot}, we observe the medians
for uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications is smaller than the range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications.

% Compression

In terms of compression, LZ4 results in the lower medians for schema-driven
binary serialization specifications while GZIP results in the lower median for
schema-less binary serialization specifications.  However, compression is not
space-efficient in terms of the median for both schema-driven and schema-less
binary serialization specifications.  Additionally, the use of LZ4 for
schema-less binary serialization specifications exhibits upper outliers.  While
compression does not contribute to space-efficiency, it reduces the range
between the upper and lower whiskers and inter-quartile range for schema-driven
binary serialization specifications.  In particular, the compression formats
with the smaller range between the upper and lower whiskers for schema-driven
binary serialization specifications are GZIP and LZMA, the compression format
with the smaller inter-quartile range for schema-driven binary serialization
specifications is LZMA, and the compression format with the smaller range
between the upper and lower whiskers and the smaller inter-quartile range for
schema-less binary serialization specifications is LZ4.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less binary
serialization specifications and that compression does not contribute to
space-efficiency in comparison to both uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/travisnotifications.tex <==
In \autoref{fig:benchmark-travisnotifications-boxplot}, we observe the medians
for uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications is smaller than the range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications. The low outlier for
uncompressed schema-less binary serialization specification represents the
space-efficiency of FlexBuffers \cite{flexbuffers} given its string
de-duplication features.

% Compression

In terms of compression, LZMA results in the lower medians for schema-driven
binary serialization specifications while GZIP results in the lower median for
schema-less binary serialization specifications.  Additionally, GZIP, LZ4 and
LZMA are space-efficient in terms of the median in comparison to both
uncompressed schema-driven and schema-less binary serialization specifications.
However, the use of GZIP, LZ4 and LZMA for schema-driven binary serialization
specifications and schema-less binary serialization specifications exhibits
upper outliers.  Nevertheless, compression reduces the range between the upper
and lower whiskers and inter-quartile range for both schema-driven and
schema-less binary serialization specifications.  In particular, the
compression format with the smaller range between the upper and lower whiskers
and the smaller inter-quartile range for schema-driven binary serialization
specifications is LZMA, and the compression formats with the smaller range
between the upper and lower whiskers for schema-less binary serialization
specifications are LZ4 and LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less
binary serialization specifications and that all the considered compression
formats are space-efficient in comparison to uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/tslintbasic.tex <==
In \autoref{fig:benchmark-tslintbasic-boxplot}, we observe the medians for
uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers of uncompressed schema-driven binary
serialization specifications is smaller than the range between the upper and lower
whiskers of uncompressed schema-less binary serialization specifications.  However,
the inter-quartile range of both both uncompressed schema-driven and
schema-less binary serialization specifications is similar.

% Compression

In terms of compression, GZIP and LZ4 result in the lower medians for
schema-driven binary serialization specifications while GZIP results in the
lower median for schema-less binary serialization specifications.  However,
compression is not space-efficient in terms of the median for both
schema-driven and schema-less binary serialization specifications.
Additionally, the use of GZIP, LZ4 and LZMA for schema-driven binary
serialization specifications exhibits upper outliers.  While compression does
not contribute to space-efficiency, it reduces the range between the upper and
lower whiskers and inter-quartile range for both schema-driven and schema-less
binary serialization specifications.  In particular, the compression format
with the smaller range between the upper and lower whiskers for schema-driven
binary serialization specifications is LZMA, the compression formats with the
smaller inter-quartile range for schema-driven binary serialization
specifications are GZIP and LZMA, the compression format with the smaller range
between the upper and lower whiskers for schema-less binary serialization
specifications is GZIP, and the compression formats with the smaller
inter-quartile range for schema-less binary serialization specifications are
LZ4 and LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less binary
serialization specifications and that compression does not contribute to
space-efficiency in comparison to both uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/tslintextend.tex <==
In \autoref{fig:benchmark-tslintextend-boxplot}, we observe the medians for
uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-less binary serialization specifications is smaller than the range
between the upper and lower whiskers and the inter-quartile range of
uncompressed schema-driven binary serialization specifications. However, their
respective quartiles overlap.

% Compression

In terms of compression, GZIP results in the lower median for both
schema-driven and schema-less binary serialization specifications.  However,
compression is not space-efficient in terms of the median for both
schema-driven and schema-less binary serialization specifications.  While
compression does not contribute to space-efficiency, it reduces the range
between the upper and lower whiskers and inter-quartile range for schema-driven
binary serialization specifications.  In particular, the compression format
with the smaller range between the upper and lower whiskers for schema-driven
binary serialization specifications is LZMA, the compression formats with the
smaller inter-quartile range for schema-driven binary serialization
specifications are GZIP and LZMA, and the compression format with the smaller
range between the upper and lower whiskers for schema-less binary serialization
specifications is LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less
binary serialization specifications and that compression does not contribute to
space-efficiency in comparison to both uncompressed schema-driven and
schema-less binary serialization specifications.


==> boxplots/tslintmulti.tex <==
In \autoref{fig:benchmark-tslintmulti-boxplot}, we observe the medians for
uncompressed schema-driven binary serialization specifications to be smaller in
comparison to uncompressed schema-less binary serialization specifications.  The range
between the upper and lower whiskers of uncompressed schema-driven binary
serialization specifications is smaller than the range between the upper and lower
whiskers of uncompressed schema-less binary serialization specifications.  However,
the inter-quartile range of both both uncompressed schema-driven and
schema-less binary serialization specifications is similar.

% Compression

In terms of compression, GZIP results in the lower median for both
schema-driven and schema-less binary serialization specifications.  However,
compression is not space-efficient in terms of the median for both
schema-driven and schema-less binary serialization specifications.
Additionally, the use of GZIP, LZ4 and LZMA for schema-driven binary
serialization specifications exhibits upper outliers.  While compression does
not contribute to space-efficiency, it reduces the range between the upper and
lower whiskers and inter-quartile range for both schema-driven and schema-less
binary serialization specifications.  In particular, the compression format
with the smaller range between the upper and lower whiskers for schema-driven
binary serialization specifications is LZMA, the compression formats with the
smaller inter-quartile range for schema-driven binary serialization
specifications are GZIP and LZMA, the compression format with the smaller range
between the upper and lower whiskers for schema-less binary serialization
specifications is GZIP, and the compression formats with the smaller
inter-quartile range for schema-less binary serialization specifications are
GZIP and LZMA.

% Conclusion

Overall, \we conclude that uncompressed schema-driven binary serialization
specifications are space-efficient in comparison to uncompressed schema-less
binary serialization specifications and that compression does not contribute to
space-efficiency in comparison to both uncompressed schema-driven and
schema-less binary serialization specifications.


==> discussions/circleciblank.tex <==
The smallest bit-string is produced by both ASN.1 PER Unaligned \cite{asn1-per}
and Apache Avro \cite{avro} (4 bytes), closely followed by Protocol Buffers
\cite{protocolbuffers} (5 bytes) and Cap'n Proto Packed Encoding
\cite{capnproto} (6 bytes). These serialization specifications are
schema-driven and with the exception of Cap'n Proto Packed Encoding, which
occupies the fourth place, they are also sequential \cite{viotti2022survey}. Conversely, the
largest bit-string is produced by Cap'n Proto Binary Encoding \cite{capnproto}
(24 bytes), followed by FlatBuffers \cite{flatbuffers} (20 bytes) and both BSON
\cite{bson} and FlexBuffers \cite{flexbuffers} (18 bytes).  With the exception
of BSON, the binary serialization specifications that produced the largest
bit-strings are pointer-based \cite{viotti2022survey}. In comparison to JSON \cite{ECMA-404}
(14 bytes), binary serialization achieves a \textbf{3.5x} size reduction in the
best case for this input document. However, 5 out of the 14 JSON-compatible
binary serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: Cap'n Proto Binary Encoding \cite{capnproto}, FlatBuffers
\cite{flatbuffers}, BSON \cite{bson}, FlexBuffers \cite{flexbuffers} and Smile
\cite{smile}. These binary serialization specifications are either schema-less
or schema-driven and pointer-based.

For this Tier 1 NNF document, the best performing schema-driven serialization
specification achieves a \textbf{2.5x} size reduction compared to the best
performing schema-less serialization specification: CBOR \cite{RFC7049} and
MessagePack \cite{messagepack} (10 bytes). As shown in
\autoref{table:benchmark-stats-circleciblank}, uncompressed schema-driven
specifications provide smaller \emph{average} and \emph{median} bit-strings
than uncompressed schema-less specifications. However, as highlighted by the
\emph{range} and \emph{standard deviation}, uncompressed schema-driven
specifications exhibit higher size reduction variability depending on the
schema language capabilities and implemented size optimizations. With the
exception of the pointer-based binary serialization specifications Cap'n Proto
Binary Encoding \cite{capnproto} and FlatBuffers \cite{flatbuffers}, the
selection of schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification only achieves a \textbf{1.5x} size reduction
compared to the best performing pointer-based serialization specification:
Cap'n Proto Packed Encoding \cite{capnproto} (6 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} do not result in positive
gains for any case due to the overhead of encoding the dictionary data
structures and the low redundancy of the input data. The best performing
uncompressed binary serialization specification achieves a \textbf{8.2x} size
reduction compared to the best performing compression format for JSON: LZ4 (33
bytes).


==> discussions/circlecimatrix.tex <==
The smallest bit-string is produced by Apache Avro \cite{avro} (15 bytes),
followed by ASN.1 PER Unaligned \cite{asn1-per} (18 bytes) and Protocol Buffers
\cite{protocolbuffers} (26 bytes). The binary serialization specifications that
produced the smallest bit-strings are schema-driven and sequential \cite{viotti2022survey}.
Conversely, the largest bit-string is produced by FlexBuffers
\cite{flexbuffers} (157 bytes), BSON \cite{bson} (136 bytes) and FlatBuffers
\cite{flatbuffers} (104 bytes). With the exception of BSON, the binary
serialization specifications that produced the largest bit-strings are pointer-based
\cite{viotti2022survey}.  In comparison to JSON \cite{ECMA-404} (95 bytes), binary
serialization achieves a \textbf{6.3x} size reduction in the best case for this
input document. However, 4 out of the 14 JSON-compatible binary serialization
specifications listed in \autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: Cap'n Proto Binary Encoding \cite{capnproto}, FlatBuffers
\cite{flatbuffers}, BSON \cite{bson} and FlexBuffers \cite{flexbuffers}. These
binary serialization specifications are either schema-less or schema-driven and
pointer-based.

For this Tier 1 NNN document, the best performing schema-driven serialization
specification achieves a \textbf{4.8x} size reduction compared to the best performing
schema-less serialization specification: CBOR \cite{RFC7049} and MessagePack
\cite{messagepack} (72 bytes).  As shown in
\autoref{table:benchmark-stats-circlecimatrix}, uncompressed schema-driven
specifications provide smaller \emph{average} and \emph{median} bit-strings than
uncompressed schema-less specifications. However, as highlighted by the \emph{range}
and \emph{standard deviation}, uncompressed schema-driven specifications exhibit
higher size reduction variability depending on the schema language capabilities
and implemented size optimizations. With the exception of the pointer-based
binary serialization specifications Cap'n Proto Binary Encoding \cite{capnproto} and
FlatBuffers \cite{flatbuffers}, the selection of schema-driven serialization
specifications listed in \autoref{table:benchmark-specifications-schema-driven} produce
bit-strings that are equal to or smaller than their schema-less counterparts
listed in \autoref{table:benchmark-specifications-schema-less}.  The best performing
sequential serialization specification achieves a \textbf{2.4x} size reduction
compared to the best performing pointer-based serialization specification: Cap'n Proto
Packed Encoding \cite{capnproto} (36 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
the bit-strings produced by Cap'n Proto Binary Encoding \cite{capnproto},
FlatBuffers \cite{flatbuffers}, BSON \cite{bson} and FlexBuffers
\cite{flexbuffers}. The best performing uncompressed binary serialization
specification achieves a \textbf{6.6x} size reduction compared to the best
performing compression format for JSON: GZIP \cite{RFC1952} (99 bytes).


==> discussions/commitlint.tex <==
The smallest bit-string is produced by Apache Avro \cite{avro} (40 bytes),
followed by ASN.1 PER Unaligned \cite{asn1-per} (50 bytes) and Apache Thrift
\cite{slee2007thrift} (59 bytes).  The binary serialization specifications that
produced the smallest bit-strings are schema-driven and sequential \cite{viotti2022survey}.
Conversely, the largest bit-string is produced by FlatBuffers
\cite{flatbuffers} (156 bytes), Cap'n Proto Binary Encoding \cite{capnproto}
(152 bytes) and BSON \cite{bson} (147 bytes). With the exception of BSON, the
binary serialization specifications that produced the largest bit-strings are
pointer-based \cite{viotti2022survey}.  In comparison to JSON \cite{ECMA-404} (96 bytes),
binary serialization achieves a \textbf{2.4x} size reduction in the best case
for this input document. However, 3 out of the 14 JSON-compatible binary
serialization specifications listed in \autoref{table:benchmark-specifications-schema-driven}
and \autoref{table:benchmark-specifications-schema-less} result in bit-strings that
are larger than JSON: Cap'n Proto Binary Encoding \cite{capnproto}, FlatBuffers
\cite{flatbuffers} and BSON \cite{bson}. These binary serialization specifications are
either schema-less or schema-driven and pointer-based.

For this Tier 1 TRN document, the best performing schema-driven serialization
specification only achieves a \textbf{1.8x} size reduction compared to the best
performing schema-less serialization specification: CBOR \cite{RFC7049} and
MessagePack \cite{messagepack} (74 bytes).  As shown in
\autoref{table:benchmark-stats-commitlint}, uncompressed schema-driven specifications
provide smaller \emph{average} and \emph{median} bit-strings than uncompressed
schema-less specifications. However, as highlighted by the \emph{range} and
\emph{standard deviation}, uncompressed schema-driven specifications exhibit higher
size reduction variability depending on the expressiveness of the schema
language (i.e. how the language constructs allow you to model the data) and the
size optimizations devised by its authors. With the exception of the
pointer-based binary serialization specifications Cap'n Proto Binary Encoding
\cite{capnproto}, Cap'n Proto Packed Encoding \cite{capnproto} and FlatBuffers
\cite{flatbuffers}, the selection of schema-driven serialization specifications listed
in \autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification achieves a \textbf{1.9x} size reduction compared to the
best performing pointer-based serialization specification: Cap'n Proto Packed Encoding
\cite{capnproto} (76 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
all the bit-strings except the ones produced by Apache Avro \cite{avro} and
FlexBuffers \cite{flexbuffers}. The best performing uncompressed binary
serialization specification achieves a \textbf{2x} size reduction compared to
the best performing compression format for JSON: GZIP \cite{RFC1952} (80
bytes).


==> discussions/commitlintbasic.tex <==
The smallest bit-string is produced by Protocol Buffers \cite{protocolbuffers}
(0 bytes), closely followed by both ASN.1 PER Unaligned \cite{asn1-per} and
Apache Avro \cite{avro} (1 byte), and Apache Thrift \cite{slee2007thrift} (2
bytes). Protocol Buffers \cite{protocolbuffers} achieves a zero byte-size as
the input document consists of the boolean value \emph{false}, which Protocol
Buffers represents by not encoding the corresponding field. The binary
serialization specifications that produced the smallest bit-strings are schema-driven
and sequential \cite{viotti2022survey}. Conversely, the larges bit-string is produced by
FlexBuffers \cite{flexbuffers} (152 bytes) followed by UBJSON \cite{ubjson}
(137 bytes) and BSON \cite{bson} (133 bytes).  The binary serialization specifications
that produced the largest bit-strings are schema-less.  With the exception of
FlexBuffers, the binary serialization specifications that produced the largest
bit-strings are also sequential \cite{viotti2022survey}.  In comparison to JSON
\cite{ECMA-404} (25 bytes), binary serialization achieves 0 bytes in the best
case for this input document, the maximal possible size reduction.
Additionally, none of the 14 JSON-compatible binary serialization specifications
listed in \autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON. However, the FlexBuffers \cite{flexbuffers} schema-less
pointer-based serialization specification result in a bit-string that is equal in size
to JSON.

For this Tier 1 BNF document, the best performing schema-less serialization
specifications are CBOR \cite{RFC7049} and MessagePack \cite{messagepack} (17 bytes).
As shown in \autoref{table:benchmark-stats-commitlintbasic}, uncompressed
schema-driven specifications provide smaller \emph{average} and \emph{median}
bit-strings than uncompressed schema-less specifications. However, as highlighted by
the \emph{range} and \emph{standard deviation}, uncompressed schema-driven
specifications exhibit higher size reduction variability depending on the
expressiveness of the schema language (i.e. how the language constructs allow
you to model the data) and the size optimizations devised by its authors. With
the exception of the pointer-based binary serialization specifications Cap'n Proto
Binary Encoding \cite{capnproto} and FlatBuffers \cite{flatbuffers}, the
selection of schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing
pointer-based serialization specification is Cap'n Proto Packed Encoding
\cite{capnproto} (6 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} do not result in positive
gains for any bit-string due to the overhead of encoding the dictionary data
structures and the low redundancy of the input data. The best performing
compression format for JSON is LZ4 (44 bytes).


==> discussions/epr.tex <==
The smallest bit-string is produced by Apache Avro \cite{avro} (195 bytes)
followed by ASN.1 PER Unaligned \cite{asn1-per} (231 bytes) and Protocol
Buffers \cite{protocolbuffers} (247 bytes). The binary serialization specifications
that produced the smallest bit-strings are schema-driven and sequential
\cite{viotti2022survey}. Conversely, the largest bit-string is produced by BSON \cite{bson}
(564 bytes) followed by Cap'n Proto Binary Encoding \cite{capnproto} (536
bytes) and FlatBuffers \cite{flatbuffers} (504 bytes).  With the exception of
BSON, the binary serialization specifications that produced the largest bit-strings
are schema-driven and pointer-based \cite{viotti2022survey}.  In comparison to JSON
\cite{ECMA-404} (520 bytes), binary serialization achieves a \textbf{2.6x} size
reduction in the best case for this input document.  However, 2 out of the 14
JSON-compatible binary serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: Cap'n Proto Binary Encoding \cite{capnproto} and BSON
\cite{bson}. These binary serialization specifications are either schema-less or
schema-driven and pointer-based.

For this Tier 2 TRN document, the best performing schema-driven serialization
specification only achieves a \textbf{1.8x} size reduction compared to the best
performing schema-less serialization specification: Smile \cite{smile} (356 bytes).
As shown in \autoref{table:benchmark-stats-epr}, uncompressed schema-driven
specifications provide smaller \emph{average} and \emph{median} bit-strings than
uncompressed schema-less specifications. However, as highlighted by the \emph{range}
and \emph{standard deviation}, uncompressed schema-driven specifications exhibit
higher size reduction variability depending on the expressiveness of the schema
language (i.e. how the language constructs allow you to model the data) and the
size optimizations devised by its authors. With the exception of the
pointer-based binary serialization specifications Cap'n Proto Binary Encoding
\cite{capnproto} and FlatBuffers \cite{flatbuffers}, the selection of
schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification only achieves a \textbf{1.6x} size reduction compared to
the best performing pointer-based serialization specification: Cap'n Proto Packed
Encoding \cite{capnproto} (318 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
all bit-strings. The best performing uncompressed binary serialization
specification achieves a \textbf{1.3x} size reduction compared to the best
performing compression format for JSON: GZIP \cite{RFC1952} (264 bytes).


==> discussions/eslintrc.tex <==
The smallest bit-string is produced by ASN.1 PER Unaligned \cite{asn1-per} (65
bytes) followed by Apache Avro \cite{avro} (100 bytes) and Cap'n Proto Packed
Encoding \cite{capnproto} (131 bytes). These serialization specifications are
schema-driven and with the exception of Cap'n Proto Packed Encoding, which
occupies the third place, they are also sequential \cite{viotti2022survey}.  Conversely, the
largest bit-string is produced by FlexBuffers \cite{flexbuffers} (1201 bytes)
followed by BSON \cite{bson} (1184 bytes) and UBJSON \cite{ubjson} (1070
bytes). The binary serialization specifications that produced the largest bit-strings
are schema-less and with the exception of FlexBuffers, they are also sequential
\cite{viotti2022survey}.  In comparison to JSON \cite{ECMA-404} (1141 bytes), binary
serialization achieves a \textbf{17.5x} size reduction in the best case for
this input document.  Similar large size reductions are observed in JSON
documents whose content is dominated by \emph{boolean} and \emph{numeric}
values.  However, 2 out of the 14 JSON-compatible binary serialization specifications
listed in \autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: BSON \cite{bson} and FlexBuffers \cite{flexbuffers}. These
binary serialization specifications are schema-less.

For this Tier 3 NRF document, the best performing schema-driven serialization
specification achieves a \textbf{14.9x} size reduction compared to the best performing
schema-less serialization specification: MessagePack \cite{messagepack} (971 bytes).
As shown in \autoref{table:benchmark-stats-eslintrc}, uncompressed
schema-driven specifications provide smaller \emph{average} and \emph{median}
bit-strings than uncompressed schema-less specifications. The entire selection of
schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification achieves a \textbf{2x} size reduction compared to the best
performing pointer-based serialization specification: Cap'n Proto Packed Encoding
\cite{capnproto} (131 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
all the bit-strings except the one produced by ASN.1 PER Unaligned
\cite{asn1-per}. The best performing uncompressed binary serialization
specification achieves a \textbf{7.5x} size reduction compared to the best
performing compression format for JSON: GZIP \cite{RFC1952} (488 bytes).


==> discussions/esmrc.tex <==
The smallest bit-string is produced by ASN.1 PER Unaligned \cite{asn1-per} (12
bytes), followed by Apache Avro \cite{avro} (16 bytes) and Protocol Buffers
\cite{protocolbuffers} (23 bytes). The binary serialization specifications that
produced the smallest bit-strings are schema-driven and sequential \cite{viotti2022survey}.
Conversely, the largest bit-string is produced by BSON \cite{bson} (96 bytes),
followed by FlexBuffers \cite{flexbuffers} (91 bytes) and FlatBuffers
\cite{flatbuffers} (80 bytes). With the exception of BSON, the binary
serialization specifications that produced the largest bit-strings are pointer-based
\cite{viotti2022survey}.  In comparison to JSON \cite{ECMA-404} (102 bytes), binary
serialization achieves a \textbf{8.5x} size reduction in the best case for this
input document.  None of the 14 JSON-compatible binary serialization specifications
listed in \autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON.

For this Tier 2 BNF document, the best performing schema-driven serialization
specification achieves a \textbf{5.3x} size reduction compared to the best performing
schema-less serialization specification: CBOR \cite{RFC7049} and MessagePack
\cite{messagepack} (64 bytes).  As shown in
\autoref{table:benchmark-stats-esmrc}, uncompressed schema-driven specifications
provide smaller \emph{average} and \emph{median} bit-strings than uncompressed
schema-less specifications. However, as highlighted by the \emph{range} and
\emph{standard deviation}, uncompressed schema-driven specifications exhibit higher
size reduction variability depending on the expressiveness of the schema
language (i.e. how the language constructs allow you to model the data) and the
size optimizations devised by its authors. With the exception of the
pointer-based binary serialization specifications Cap'n Proto Binary Encoding
\cite{capnproto} and FlatBuffers \cite{flatbuffers}, the selection of
schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification achieves a \textbf{2.9x} size reduction compared to the
best performing pointer-based serialization specification: Cap'n Proto Packed Encoding
\cite{capnproto} (35 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
the bit-strings produced by Cap'n Proto Binary Encoding \cite{capnproto},
FlatBuffers \cite{flatbuffers} and JSON \cite{ECMA-404}. The best performing
uncompressed binary serialization specification achieves a \textbf{8.4x} size
reduction compared to the best performing compression format for JSON: GZIP
\cite{RFC1952} (101 bytes).


==> discussions/geojson.tex <==
In this exceptional case, the smallest bit-strings for this input document are
produced by the schema-less sequential specifications MessagePack
\cite{messagepack} (162 bytes) and CBOR \cite{RFC7049} (172 bytes), followed by
the schema-driven sequential specification ASN.1 PER Unaligned \cite{asn1-per}
(205 bytes). In comparison to other input documents, this input document
defines poly-dimensional JSON \cite{ECMA-404} arrays, which the schema-driven
binary serialization specifications from the selection do not encode in a
space-efficient manner. Similarly to other cases, the largest bit-string is
produced by FlatBuffers \cite{flatbuffers} (680 bytes), followed by BSON
\cite{bson} (456 bytes) and Cap'n Proto Binary Encoding \cite{capnproto} (448
bytes). With the exception of BSON, the binary serialization specifications
that produced the largest bit-strings are pointer-based \cite{viotti2022survey}.  In
comparison to JSON \cite{ECMA-404} (190 bytes), binary serialization only
achieves a \textbf{1.1x} size reduction in the best case for this input
document. With the exception of the schema-less sequential MessagePack
\cite{messagepack} and CBOR \cite{RFC7049} binary serialization specifications,
all the other JSON-compatible binary serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that
are larger than JSON.

For this Tier 2 NRN document, the smaller bit-string is produced by a
schema-less specification.  However, the best performing schema-less serialization
specification only achieves a \textbf{1.2x} size reduction compared to the best
performing schema-driven serialization specification: ASN.1 PER Unaligned
\cite{asn1-per} (205 bytes).  As shown in
\autoref{table:benchmark-stats-geojson}, uncompressed schema-less specifications
provide smaller \emph{average} and \emph{median} bit-strings than uncompressed
schema-driven specifications. Additionally, as highlighted by the \emph{range} and
\emph{standard deviation}, uncompressed schema-driven specifications exhibit higher
size reduction variability depending on the expressiveness of the schema
language (i.e. how the language constructs allow you to model the data) and the
size optimizations devised by its authors.  The schema-less and sequential
specifications CBOR \cite{RFC7049} and MessagePack \cite{messagepack} produce
bit-strings that are smaller to all their schema-driven counterparts listed in
\autoref{table:benchmark-specifications-schema-driven}.  The best performing
sequential serialization specification only achieves a \textbf{1.4x} size reduction
compared to the best performing pointer-based serialization specification: Cap'n Proto
Packed Encoding \cite{capnproto} (228 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
all bit-strings. The best performing compression format for JSON, LZMA (116
bytes), achieve a \textbf{1.3x} size reduction compared to the best performing
uncompressed binary serialization specification.


==> discussions/githubfundingblank.tex <==
The smallest bit-string is produced by both ASN.1 PER Unaligned \cite{asn1-per}
and Apache Avro \cite{avro} (16 bytes), closely followed by Protocol Buffers
\cite{protocolbuffers} (17 bytes) and Apache Thrift \cite{slee2007thrift} (18
bytes). The binary serialization specifications that produced the smallest bit-strings
are schema-driven and sequential \cite{viotti2022survey}.  Conversely, the largest bit-string
is produced by FlexBuffers \cite{flexbuffers} (152 bytes), followed by UBJSON
\cite{ubjson} (137 bytes) and BSON \cite{bson} (133 bytes). The binary
serialization specifications that produced the largest bit-strings are schema-less and
with the exception of FlexBuffers, they are also sequential \cite{viotti2022survey}.  In
comparison to JSON \cite{ECMA-404} (183 bytes), binary serialization achieves a
\textbf{11.4x} size reduction in the best case for this input document.
Similar large size reductions are observed in JSON documents whose content is
dominated by \emph{boolean} and \emph{numeric} values.  None of the 14
JSON-compatible binary serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON.

For this Tier 2 BRF document, the best performing schema-driven serialization
specification achieves a \textbf{7.7x} size reduction compared to the best performing
schema-less serialization specification: CBOR \cite{RFC7049} and MessagePack
\cite{messagepack} (124 bytes).  As shown in
\autoref{table:benchmark-stats-githubfundingblank}, uncompressed schema-driven
specifications provide smaller \emph{average} and \emph{median} bit-strings than
uncompressed schema-less specifications. However, as highlighted by the \emph{range}
and \emph{standard deviation}, uncompressed schema-driven specifications exhibit
higher size reduction variability depending on the expressiveness of the schema
language (i.e. how the language constructs allow you to model the data) and the
size optimizations devised by its authors.  The entire selection of
schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification only achieves a \textbf{1.5x} size reduction compared to
the best performing pointer-based serialization specification: Cap'n Proto Packed
Encoding \cite{capnproto} (25 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
the bit-strings produced by JSON \cite{ECMA-404}, BSON \cite{bson}, CBOR
\cite{RFC7049}, FlexBuffers \cite{flexbuffers} and UBJSON \cite{ubjson}. The
best performing uncompressed binary serialization specification achieves a
\textbf{8.3x} size reduction compared to the best performing compression format
for JSON: GZIP \cite{RFC1952} (134 bytes).


==> discussions/githubworkflow.tex <==
The smallest bit-string is produced by ASN.1 PER Unaligned \cite{asn1-per} (165
bytes), closely followed by Apache Avro \cite{avro} (167 bytes) and Apache
Thrift \cite{slee2007thrift} (187 bytes).  The binary serialization specifications
that produced the smallest bit-strings are schema-driven and sequential
\cite{viotti2022survey}. Conversely, the largest bit-string is produced by Cap'n Proto Binary
Encoding \cite{capnproto} (464 bytes), followed by FlatBuffers
\cite{flatbuffers} (440 bytes) and BSON \cite{bson} (411 bytes).  With the
exception of BSON, the binary serialization specifications that produced the largest
bit-strings are schema-driven and pointer-based \cite{viotti2022survey}.  In comparison to
JSON \cite{ECMA-404} (356 bytes), binary serialization achieves a \textbf{2.1x}
size reduction in the best case for this input document.  However, 4 out of the
14 JSON-compatible binary serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: Cap'n Proto Binary Encoding \cite{capnproto}, FlatBuffers
\cite{flatbuffers}, BSON \cite{bson} and FlexBuffers \cite{flexbuffers}. These
binary serialization specifications are either schema-less or schema-driven and
pointer-based.

For this Tier 2 TNN document, the best performing schema-driven serialization
specification only achieves a \textbf{1.7x} size reduction compared to the best
performing schema-less serialization specification: MessagePack \cite{messagepack} and
Smile \cite{smile} (287 bytes).  As shown in
\autoref{table:benchmark-stats-githubworkflow}, uncompressed schema-driven
specifications provide smaller \emph{average} and \emph{median} bit-strings than
uncompressed schema-less specifications. However, as highlighted by the \emph{range}
and \emph{standard deviation}, uncompressed schema-driven specifications exhibit
higher size reduction variability depending on the expressiveness of the schema
language (i.e. how the language constructs allow you to model the data) and the
size optimizations devised by its authors. With the exception of the
pointer-based binary serialization specifications Cap'n Proto Binary Encoding
\cite{capnproto} and FlatBuffers \cite{flatbuffers}, the selection of
schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification only achieves a \textbf{1.4x} size reduction compared to
the best performing pointer-based serialization specification: Cap'n Proto Packed
Encoding \cite{capnproto} (242 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
all bit-strings. The best performing uncompressed binary serialization
specification achieves a \textbf{1.3x} size reduction compared to the best
performing compression format for JSON: GZIP \cite{RFC1952} (228 bytes).


==> discussions/gruntcontribclean.tex <==
The smallest bit-string is produced by ASN.1 PER Unaligned \cite{asn1-per} (13
bytes), followed by Apache Avro \cite{avro} (16 bytes) and Protocol Buffers
\cite{protocolbuffers} (20 bytes). The binary serialization specifications that
produced the smallest bit-strings are schema-driven and sequential \cite{viotti2022survey}.
Conversely, the largest bit-string is produced by FlatBuffers
\cite{flatbuffers} (116 bytes), followed by BSON \cite{bson} (105 bytes) and
Cap'n Proto Binary Encoding \cite{capnproto} (96 bytes).  With the exception of
BSON, the binary serialization specifications that produced the largest bit-strings
are schema-driven and pointer-based \cite{viotti2022survey}.  In comparison to JSON
\cite{ECMA-404} (93 bytes), binary serialization achieves a \textbf{7.1x} size
reduction in the best case for this input document.  However, 4 out of the 14
JSON-compatible binary serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: Cap'n Proto Binary Encoding \cite{capnproto}, FlatBuffers
\cite{flatbuffers}, BSON \cite{bson} and FlexBuffers \cite{flexbuffers}. These
binary serialization specifications are either schema-less or schema-driven and
pointer-based.

For this Tier 1 TRF document, the best performing schema-driven serialization
specification achieves a \textbf{4.6x} size reduction compared to the best performing
schema-less serialization specification: CBOR \cite{RFC7049} and MessagePack
\cite{messagepack} (60 bytes).  As shown in
\autoref{table:benchmark-stats-gruntcontribclean}, uncompressed schema-driven
specifications provide smaller \emph{average} and \emph{median} bit-strings than
uncompressed schema-less specifications. However, as highlighted by the \emph{range}
and \emph{standard deviation}, uncompressed schema-driven specifications exhibit
higher size reduction variability depending on the expressiveness of the schema
language (i.e. how the language constructs allow you to model the data) and the
size optimizations devised by its authors. With the exception of the
pointer-based binary serialization specifications Cap'n Proto Binary Encoding
\cite{capnproto} and FlatBuffers \cite{flatbuffers}, the selection of
schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification achieves a \textbf{3x} size reduction compared to the best
performing pointer-based serialization specification: Cap'n Proto Packed Encoding
\cite{capnproto} (39 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
the bit-strings produced by Cap'n Proto Binary Encoding \cite{capnproto},
FlatBuffers \cite{flatbuffers} and BSON \cite{bson}.  The best performing
uncompressed binary serialization specification achieves a \textbf{7.2x} size
reduction compared to the best performing compression format for JSON: GZIP
\cite{RFC1952} (94 bytes).


==> discussions/imageoptimizerwebjob.tex <==
The smallest bit-string is produced by ASN.1 PER Unaligned \cite{asn1-per} (21
bytes), closely followed by Protocol Buffers \cite{protocolbuffers} (23 bytes)
and Apache Avro \cite{avro} (24 bytes).  The binary serialization specifications that
produced the smallest bit-strings are schema-driven and sequential \cite{viotti2022survey}.
Conversely, the largest bit-string is produced by BSON \cite{bson} (102 bytes),
closely followed by FlatBuffers \cite{flatbuffers} (100 bytes) and Cap'n Proto
Binary Encoding \cite{capnproto} (96 bytes).  With the exception of BSON, the
binary serialization specifications that produced the largest bit-strings are
schema-driven and pointer-based \cite{viotti2022survey}.  In comparison to JSON
\cite{ECMA-404} (82 bytes), binary serialization achieves a \textbf{3.9x} size
reduction in the best case for this input document.  However, 4 out of the 14
JSON-compatible binary serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: Cap'n Proto Binary Encoding \cite{capnproto}, FlatBuffers
\cite{flatbuffers}, BSON \cite{bson} and FlexBuffers \cite{flexbuffers}. These
binary serialization specifications are either schema-less or schema-driven and
pointer-based.

For this Tier 1 TNN document, the best performing schema-driven serialization
specification achieves a \textbf{2.9x} size reduction compared to the best performing
schema-less serialization specification: CBOR \cite{RFC7049} and MessagePack
\cite{messagepack} (61 bytes).  As shown in
\autoref{table:benchmark-stats-imageoptimizerwebjob}, uncompressed
schema-driven specifications provide smaller \emph{average} and \emph{median}
bit-strings than uncompressed schema-less specifications. However, as highlighted by
the \emph{range} and \emph{standard deviation}, uncompressed schema-driven
specifications exhibit higher size reduction variability depending on the
expressiveness of the schema language (i.e. how the language constructs allow
you to model the data) and the size optimizations devised by its authors. With
the exception of the pointer-based binary serialization specifications Cap'n Proto
Binary Encoding \cite{capnproto} and FlatBuffers \cite{flatbuffers}, the
selection of schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification achieves a \textbf{2x} size reduction compared to the best
performing pointer-based serialization specification: Cap'n Proto Packed Encoding
\cite{capnproto} (44 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
the bit-strings produced by Cap'n Proto Binary Encoding \cite{capnproto} and
FlatBuffers \cite{flatbuffers}. The best performing uncompressed binary
serialization specification achieves a \textbf{4.1x} size reduction compared to
the best performing compression format for JSON: GZIP \cite{RFC1952} (88
bytes).


==> discussions/jsonereversesort.tex <==
The smallest bit-string is produced by Apache Avro \cite{avro} (11 bytes),
followed by ASN.1 PER Unaligned \cite{asn1-per} (15 bytes) and Protocol Buffers
\cite{protocolbuffers} (21 bytes). The binary serialization specifications that
produced the smallest bit-strings are schema-driven and sequential \cite{viotti2022survey}.
Conversely, the largest bit-string is produced by Cap'n Proto Binary Encoding
\cite{capnproto} (240 bytes), followed by FlatBuffers \cite{flatbuffers} (136
bytes) and BSON \cite{bson} (121 bytes).  With the exception of BSON, the
binary serialization specifications that produced the largest bit-strings are
schema-driven and pointer-based \cite{viotti2022survey}.  In comparison to JSON
\cite{ECMA-404} (86 bytes), binary serialization achieves a \textbf{7.8x} size
reduction in the best case for this input document.  However, 4 out of the 14
JSON-compatible binary serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: Cap'n Proto Binary Encoding \cite{capnproto}, FlatBuffers
\cite{flatbuffers}, BSON \cite{bson} and FlexBuffers \cite{flexbuffers}. These
binary serialization specifications are either schema-less or schema-driven and
pointer-based.

For this Tier 1 NRN document, the best performing schema-driven serialization
specification achieves a \textbf{4.7x} size reduction compared to the best performing
schema-less serialization specification: CBOR \cite{RFC7049} and MessagePack
\cite{messagepack} (52 bytes).  As shown in
\autoref{table:benchmark-stats-jsonereversesort}, uncompressed schema-driven
specifications provide smaller \emph{average} and \emph{median} bit-strings than
uncompressed schema-less specifications. However, as highlighted by the \emph{range}
and \emph{standard deviation}, uncompressed schema-driven specifications exhibit
higher size reduction variability depending on the expressiveness of the schema
language (i.e. how the language constructs allow you to model the data) and the
size optimizations devised by its authors. With the exception of the
pointer-based binary serialization specifications Cap'n Proto Binary Encoding
\cite{capnproto} and FlatBuffers \cite{flatbuffers}, the selection of
schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification achieves a \textbf{3.9x} size reduction compared to the
best performing pointer-based serialization specification: Cap'n Proto Packed Encoding
\cite{capnproto} (43 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
the bit-strings produced by Cap'n Proto Binary Encoding \cite{capnproto},
FlatBuffers \cite{flatbuffers} and BSON \cite{bson}.  The best performing
uncompressed binary serialization specification achieves a \textbf{7.8x} size
reduction compared to the best performing compression format for JSON: GZIP
\cite{RFC1952} (86 bytes).


==> discussions/jsonesort.tex <==
The smallest bit-string is produced by Apache Avro \cite{avro} (9 bytes),
closely followed by Protocol Buffers \cite{protocolbuffers} (10 bytes) and
Apache Thrift \cite{slee2007thrift} (11 bytes). The binary serialization
specifications that produced the smallest bit-strings are schema-driven and sequential
\cite{viotti2022survey}. Conversely, the largest bit-string is produced by BSON \cite{bson}
(65 bytes), followed by Cap'n Proto Binary Encoding \cite{capnproto} (48 bytes)
and FlatBuffers \cite{flatbuffers} (44 bytes). With the exception of BSON, the
binary serialization specifications that produced the largest bit-strings are
schema-driven and pointer-based \cite{viotti2022survey}.  In comparison to JSON
\cite{ECMA-404} (34 bytes), binary serialization achieves a \textbf{3.7x} size
reduction in the best case for this input document.  However, 4 out of the 14
JSON-compatible binary serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: Cap'n Proto Binary Encoding \cite{capnproto}, FlatBuffers
\cite{flatbuffers}, BSON \cite{bson} and FlexBuffers \cite{flexbuffers}. These
binary serialization specifications are either schema-less or schema-driven and
pointer-based.

For this Tier 1 NRF document, the best performing schema-driven serialization
specification achieves a \textbf{2.3x} size reduction compared to the best performing
schema-less serialization specification: CBOR \cite{RFC7049} and MessagePack
\cite{messagepack} (21 bytes).  As shown in
\autoref{table:benchmark-stats-jsonesort}, uncompressed schema-driven specifications
provide smaller \emph{average} and \emph{median} bit-strings than uncompressed
schema-less specifications. Additionally, as highlighted by the \emph{range} and
\emph{standard deviation}, uncompressed schema-less specifications exhibit higher size
reduction variability given that BSON \cite{bson} produces a notably large
bit-string. With the exception of the pointer-based binary serialization
specifications Cap'n Proto Binary Encoding \cite{capnproto} and FlatBuffers
\cite{flatbuffers}, the selection of schema-driven serialization specifications listed
in \autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification achieves a \textbf{2x} size reduction compared to the best
performing pointer-based serialization specification: Cap'n Proto Packed Encoding
\cite{capnproto} (18 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
the bit-string produced by Cap'n Proto Binary Encoding \cite{capnproto}. The
best performing uncompressed binary serialization specification achieves a
\textbf{5.8x} size reduction compared to the best performing compression format
for JSON: LZ4 (53 bytes).


==> discussions/jsonfeed.tex <==
The smallest bit-string is produced by ASN.1 PER Unaligned \cite{asn1-per} (398
bytes), closely followed by Apache Avro \cite{avro} (400 bytes) and Protocol
Buffers \cite{protocolbuffers} (413 bytes). The binary serialization specifications
that produced the smallest bit-strings are schema-driven and sequential
\cite{viotti2022survey}. Conversely, the largest bit-string is produced by FlexBuffers
\cite{flexbuffers} (598 bytes), closely followed by BSON \cite{bson} (596
bytes) and FlatBuffers \cite{flatbuffers} (584 bytes). With the exception of
BSON, the binary serialization specifications that produced the largest bit-strings
are pointer-based \cite{viotti2022survey}.  In comparison to JSON \cite{ECMA-404} (573 bytes),
binary serialization only achieves a \textbf{1.4x} size reduction in the best
case for this input document.  Additionally, 3 out of the 14 JSON-compatible
binary serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: FlatBuffers \cite{flatbuffers}, BSON \cite{bson} and
FlexBuffers \cite{flexbuffers}. These binary serialization specifications are either
schema-less or schema-driven and pointer-based.

For this Tier 2 TNF document, the best performing schema-driven serialization
specification only achieves a \textbf{1.2x} size reduction compared to the best
performing schema-less serialization specification: MessagePack \cite{messagepack}
(517 bytes).  As shown in \autoref{table:benchmark-stats-jsonfeed},
uncompressed schema-driven specifications provide smaller \emph{average} and
\emph{median} bit-strings than uncompressed schema-less specifications. However, as
highlighted by the \emph{range} and \emph{standard deviation}, uncompressed
schema-driven specifications exhibit higher size reduction variability depending on
the expressiveness of the schema language (i.e. how the language constructs
allow you to model the data) and the size optimizations devised by its authors.
With the exception of the pointer-based binary serialization specifications Cap'n
Proto Binary Encoding \cite{capnproto} and FlatBuffers \cite{flatbuffers}, the
selection of schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification only achieves a \textbf{1.1x} size reduction compared to
the best performing pointer-based serialization specification: Cap'n Proto Packed
Encoding \cite{capnproto} (470 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
all bit-strings. The best performing compression format for JSON, GZIP
\cite{RFC1952} (327 bytes), achieves a \textbf{1.2x} size reduction compared to
the best performing uncompressed binary serialization specification.


==> discussions/jsonresume.tex <==
The smallest bit-string is produced by ASN.1 PER Unaligned \cite{asn1-per}
(2143 bytes), closely followed by Apache Avro \cite{avro} (2162 bytes) and
Protocol Buffers \cite{protocolbuffers} (2225 bytes). The binary serialization
specifications that produced the smallest bit-strings are schema-driven and sequential
\cite{viotti2022survey}. Conversely, the largest bit-string is produced by BSON \cite{bson}
(3283 bytes), followed by Cap'n Proto Binary Encoding \cite{capnproto} (3152
bytes) and FlatBuffers \cite{flatbuffers} (3116 bytes).  With the exception of
BSON, the binary serialization specifications that produced the largest bit-strings
are schema-driven and pointer-based \cite{viotti2022survey}.  In comparison to JSON
\cite{ECMA-404} (3048 bytes), binary serialization only achieves a
\textbf{1.4x} size reduction in the best case for this input document.
Additionally, 4 out of the 14 JSON-compatible binary serialization specifications
listed in \autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: Cap'n Proto Binary Encoding \cite{capnproto}, FlatBuffers
\cite{flatbuffers}, BSON \cite{bson} and FlexBuffers \cite{flexbuffers}. These
binary serialization specifications are either schema-less or schema-driven and
pointer-based.

For this Tier 3 TNN document, the best performing schema-driven serialization
specification only achieves a \textbf{1.2x} size reduction compared to the best
performing schema-less serialization specification: Smile \cite{smile} (2620 bytes).
As shown in \autoref{table:benchmark-stats-jsonresume}, uncompressed
schema-driven specifications provide smaller \emph{average} and \emph{median}
bit-strings than uncompressed schema-less specifications. However, as highlighted by
the \emph{range} and \emph{standard deviation}, uncompressed schema-driven
specifications exhibit higher size reduction variability depending on the
expressiveness of the schema language (i.e. how the language constructs allow
you to model the data) and the size optimizations devised by its authors. With
the exception of the pointer-based binary serialization specifications Cap'n Proto
Binary Encoding \cite{capnproto} and FlatBuffers \cite{flatbuffers}, the
selection of schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification only achieves a \textbf{1.1x} size reduction compared to
the best performing pointer-based serialization specification: Cap'n Proto Packed
Encoding \cite{capnproto} (2549 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
all bit-strings. The best performing compression format for JSON, GZIP
\cite{RFC1952} (1556 bytes), achieves a \textbf{1.3x} size reduction compared
to the best performing uncompressed binary serialization specification.


==> discussions/netcoreproject.tex <==
The smallest bit-string is produced by both ASN.1 PER Unaligned \cite{asn1-per}
and Apache Avro \cite{avro} (242 bytes), followed by Apache Thrift
\cite{slee2007thrift} (283 bytes) and Protocol Buffers \cite{protocolbuffers}
(284 bytes). The binary serialization specifications that produced the smallest
bit-strings are schema-driven and sequential \cite{viotti2022survey}.  Conversely, the largest
bit-string is produced by BSON \cite{bson} (1084 bytes), followed by UBJSON
\cite{ubjson} (1008 bytes) and CBOR \cite{RFC7049} (923 bytes).  The binary
serialization specifications that produced the largest bit-strings are schema-less and
sequential \cite{viotti2022survey}.  In comparison to JSON \cite{ECMA-404} (1049 bytes),
binary serialization achieves a \textbf{4.3x} size reduction in the best case
for this input document.  However, 1 out of the 14 JSON-compatible binary
serialization specifications listed in \autoref{table:benchmark-specifications-schema-driven}
and \autoref{table:benchmark-specifications-schema-less} result in bit-strings that
are larger than JSON: the schema-less and sequential BSON \cite{bson} binary
serialization specification.

For this Tier 3 TRN document, the best performing schema-driven serialization
specification achieves a \textbf{3.5x} size reduction compared to the best performing
schema-less serialization specification: Smile \cite{smile} (870 bytes).  As shown in
\autoref{table:benchmark-stats-netcoreproject}, uncompressed schema-driven
specifications provide smaller \emph{average} and \emph{median} bit-strings than
uncompressed schema-less specifications. However, as highlighted by the \emph{range}
and \emph{standard deviation}, uncompressed schema-driven specifications exhibit
higher size reduction variability depending on the expressiveness of the schema
language (i.e. how the language constructs allow you to model the data) and the
size optimizations devised by its authors. The entire selection of
schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification only achieves a \textbf{1.5x} size reduction compared to
the best performing pointer-based serialization specification: Cap'n Proto Packed
Encoding \cite{capnproto} (376 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
all bit-strings. The best performing uncompressed binary serialization
specification achieves a \textbf{1.6x} size reduction compared to the best
performing compression format for JSON: GZIP \cite{RFC1952} (411 bytes).


==> discussions/nightwatch.tex <==
The smallest bit-string is produced by ASN.1 PER Unaligned \cite{asn1-per} (89
bytes), followed by Apache Avro \cite{avro} (92 bytes) and Protocol Buffers
\cite{protocolbuffers} (109 bytes). The binary serialization specifications that
produced the smallest bit-strings are schema-driven and sequential \cite{viotti2022survey}.
Conversely, the largest bit-string is produced by FlexBuffers
\cite{flexbuffers} (1389 bytes), followed by BSON \cite{bson} (1327 bytes) and
UBJSON \cite{ubjson} (1268 bytes).  The binary serialization specifications that
produced the largest bit-strings are schema-less and with the exception of
FlexBuffers, they are also sequential \cite{viotti2022survey}.  In comparison to JSON
\cite{ECMA-404} (1507 bytes), binary serialization achieves a \textbf{16.9x}
size reduction in the best case for this input document.  Similar large size
reductions are observed in JSON documents whose content is dominated by
\emph{boolean} and \emph{numeric} values.  None of the 14 JSON-compatible
binary serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON.

For this Tier 3 BRF document, the best performing schema-driven serialization
specification achieves a \textbf{12.2x} size reduction compared to the best performing
schema-less serialization specification: Smile \cite{smile} (1090 bytes).  As shown in
\autoref{table:benchmark-stats-nightwatch}, uncompressed schema-driven specifications
provide smaller \emph{average} and \emph{median} bit-strings than uncompressed
schema-less specifications. However, as highlighted by the \emph{range} and
\emph{standard deviation}, uncompressed schema-driven specifications exhibit higher
size reduction variability depending on the expressiveness of the schema
language (i.e. how the language constructs allow you to model the data) and the
size optimizations devised by its authors. The entire selection of
schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification only achieves a \textbf{1.6x} size reduction compared to
the best performing pointer-based serialization specification: Cap'n Proto Packed
Encoding \cite{capnproto} (149 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
all bit-strings except the ones produced by ASN.1 PER Unaligned
\cite{asn1-per}, Apache Avro \cite{avro}, Microsoft Bond \cite{microsoft-bond},
Protocol Buffers \cite{protocolbuffers} and Apache Thrift
\cite{slee2007thrift}. The best performing uncompressed binary serialization
specification achieves a \textbf{7.2x} size reduction compared to the best
performing compression format for JSON: GZIP \cite{RFC1952} (649 bytes).


==> discussions/openweathermap.tex <==
The smallest bit-string is produced by Apache Avro \cite{avro} (148 bytes),
followed by ASN.1 PER Unaligned \cite{asn1-per} (165 bytes) and Protocol
Buffers \cite{protocolbuffers} (188 bytes).  The binary serialization specifications
that produced the smallest bit-strings are schema-driven and sequential
\cite{viotti2022survey}. Conversely, the largest bit-string is produced by FlexBuffers
\cite{flexbuffers} (660 bytes), followed by BSON \cite{bson} (480 bytes) and
UBJSON \cite{ubjson} (439 bytes). The binary serialization specifications that
produced the largest bit-strings are schema-less and with the exception of
FlexBuffers, they are also sequential \cite{viotti2022survey}.  In comparison to JSON
\cite{ECMA-404} (494 bytes), binary serialization achieves a \textbf{3.3x} size
reduction in the best case for this input document.  However, 1 out of the 14
JSON-compatible binary serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: the schema-less and pointer-based FlexBuffers
\cite{flexbuffers} binary serialization specification.

For this Tier 2 NNF document, the best performing schema-driven serialization
specification achieves a \textbf{2.5x} size reduction compared to the best performing
schema-less serialization specification: MessagePack \cite{messagepack} (382 bytes).
As shown in \autoref{table:benchmark-stats-openweathermap}, uncompressed
schema-driven specifications provide smaller \emph{average} and \emph{median}
bit-strings than uncompressed schema-less specifications. Additionally, as highlighted
by the \emph{range} and \emph{standard deviation}, uncompressed schema-less
specifications exhibit higher size reduction variability given that FlexBuffers
\cite{flexbuffers} produces a notably large bit-string. With the exception of
the pointer-based binary serialization specification FlatBuffers \cite{flatbuffers},
the selection of schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification only achieves a \textbf{1.3x} size reduction compared to
the best performing pointer-based serialization specification: Cap'n Proto Packed
Encoding \cite{capnproto} (206 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
all bit-strings except the ones produced by ASN.1 PER Unaligned
\cite{asn1-per}, Apache Avro \cite{avro}, Microsoft Bond \cite{microsoft-bond},
Cap'n Proto Packed Encoding \cite{capnproto}, Protocol Buffers
\cite{protocolbuffers} and Apache Thrift \cite{slee2007thrift}. The best
performing uncompressed binary serialization specification achieves a
\textbf{2.3x} size reduction compared to the best performing compression format
for JSON: GZIP \cite{RFC1952} (341 bytes).


==> discussions/openweatherroadrisk.tex <==
The smallest bit-string is produced by Apache Avro \cite{avro} (156 bytes),
followed by Protocol Buffers \cite{protocolbuffers} (173 bytes) and ASN.1 PER
Unaligned \cite{asn1-per} (176 bytes). The binary serialization specifications that
produced the smallest bit-strings are schema-driven and sequential \cite{viotti2022survey}.
Conversely, the largest bit-string is produced by FlexBuffers
\cite{flexbuffers} (488 bytes), followed by BSON \cite{bson} (422 bytes) and
UBJSON \cite{ubjson} (375 bytes). The binary serialization specifications that
produced the largest bit-strings are schema-less and with the exception of
FlexBuffers, they are also sequential \cite{viotti2022survey}.  In comparison to JSON
\cite{ECMA-404} (375 bytes), binary serialization achieves a \textbf{2.4x} size
reduction in the best case for this input document.  However, 2 out of the 14
JSON-compatible binary serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: BSON \cite{bson} and FlexBuffers \cite{flexbuffers}.  These
binary serialization specifications are schema-less.  Additionally, the schema-less
and sequential UBJSON \cite{ubjson} serialization specification results in a
bit-string that is equal to JSON in size.

For this Tier 2 NNN document, the best performing schema-driven serialization
specification achieves a \textbf{2x} size reduction compared to the best performing
schema-less serialization specification: Smile \cite{smile} (326 bytes).  As shown in
\autoref{table:benchmark-stats-openweatherroadrisk}, uncompressed schema-driven
specifications provide smaller \emph{average} and \emph{median} bit-strings than
uncompressed schema-less specifications. However, as highlighted by the \emph{range}
and \emph{standard deviation}, uncompressed schema-driven specifications exhibit
higher size reduction variability depending on the expressiveness of the schema
language (i.e. how the language constructs allow you to model the data) and the
size optimizations devised by its authors. With the exception of the
pointer-based binary serialization specification FlatBuffers \cite{flatbuffers}, the
selection of schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification only achieves a \textbf{1.3x} size reduction compared to
the best performing pointer-based serialization specification: Cap'n Proto Packed
Encoding \cite{capnproto} (204 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
all bit-strings. The best performing uncompressed binary serialization
specification achieves a \textbf{1.6x} size reduction compared to the best
performing compression format for JSON: GZIP \cite{RFC1952} (250 bytes).


==> discussions/packagejson.tex <==
The smallest bit-string is produced by ASN.1 PER Unaligned \cite{asn1-per}
(1498 bytes), closely followed by Apache Avro \cite{avro} (1500 bytes) and
Apache Thrift \cite{slee2007thrift} (1561 bytes). The binary serialization
specifications that produced the smallest bit-strings are schema-driven and sequential
\cite{viotti2022survey}. Conversely, the largest bit-string is produced by BSON \cite{bson}
(2386 bytes), followed by FlexBuffers \cite{flexbuffers} (2320 bytes) and
FlatBuffers \cite{flatbuffers} (2268 bytes). With the exception of BSON, the
binary serialization specifications that produced the largest bit-strings are
pointer-based \cite{viotti2022survey}.  In comparison to JSON \cite{ECMA-404} (2259 bytes),
binary serialization only achieves a \textbf{1.5x} size reduction in the best
case for this input document.  Additionally, 3 out of the 14 JSON-compatible
binary serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: FlatBuffers \cite{flatbuffers}, BSON \cite{bson} and
FlexBuffers \cite{flexbuffers}. These binary serialization specifications are either
schema-less or schema-driven and pointer-based.

For this Tier 3 TNF document, the best performing schema-driven serialization
specification only achieves a \textbf{1.3x} size reduction compared to the best
performing schema-less serialization specification: Smile \cite{smile} (1983 bytes).
As shown in \autoref{table:benchmark-stats-packagejson}, uncompressed
schema-driven specifications provide smaller \emph{average} and \emph{median}
bit-strings than uncompressed schema-less specifications. However, as highlighted by
the \emph{range} and \emph{standard deviation}, uncompressed schema-driven
specifications exhibit higher size reduction variability depending on the
expressiveness of the schema language (i.e. how the language constructs allow
you to model the data) and the size optimizations devised by its authors. With
the exception of the pointer-based binary serialization specifications Cap'n Proto
Binary Encoding \cite{capnproto} and FlatBuffers \cite{flatbuffers}, the
selection of schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification only achieves a \textbf{1.1x} size reduction compared to
the best performing pointer-based serialization specification: Cap'n Proto Packed
Encoding \cite{capnproto} (1755 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
all bit-strings. The best performing compression format for JSON, GZIP
\cite{RFC1952} (1093 bytes), achieves a \textbf{1.3x} size reduction compared
to the best performing uncompressed binary serialization specification.


==> discussions/packagejsonlintrc.tex <==
The smallest bit-string is produced by Apache Avro \cite{avro} (201 bytes),
followed by ASN.1 PER Unaligned \cite{asn1-per} (369 bytes) and Apache Thrift
\cite{slee2007thrift} (420 bytes).  The binary serialization specifications that
produced the smallest bit-strings are schema-driven and sequential \cite{viotti2022survey}.
Conversely, the largest bit-string is produced by BSON \cite{bson} (1295
bytes), followed by UBJSON \cite{ubjson} (1117 bytes) and Smile \cite{smile}
(1002 bytes). The binary serialization specifications that produced the largest
bit-strings are schema-less and sequential.  In comparison to JSON
\cite{ECMA-404} (1159 bytes), binary serialization achieves a \textbf{5.7x}
size reduction in the best case for this input document.  However, 1 out of the
14 JSON-compatible binary serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: the schema-less and sequential BSON \cite{bson} binary
serialization specification.

For this Tier 3 TRF document, the best performing schema-driven serialization
specification achieves a \textbf{4.6x} size reduction compared to the best performing
schema-less serialization specification: FlexBuffers \cite{flexbuffers} (942 bytes).
As shown in \autoref{table:benchmark-stats-packagejsonlintrc}, uncompressed
schema-driven specifications provide smaller \emph{average} and \emph{median}
bit-strings than uncompressed schema-less specifications. However, as highlighted by
the \emph{range} and \emph{standard deviation}, uncompressed schema-driven
specifications exhibit higher size reduction variability depending on the
expressiveness of the schema language (i.e. how the language constructs allow
you to model the data) and the size optimizations devised by its authors.  With
the exception of the pointer-based binary serialization specification FlatBuffers
\cite{flatbuffers}, the selection of schema-driven serialization specifications listed
in \autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification achieves a \textbf{2.5x} size reduction compared to the
best performing pointer-based serialization specification: Cap'n Proto Packed Encoding
\cite{capnproto} (519 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
all bit-strings. The best performing uncompressed binary serialization
specification achieves a \textbf{1.5x} size reduction compared to the best
performing compression format for JSON: GZIP \cite{RFC1952} (321 bytes).


==> discussions/sapcloudsdkpipeline.tex <==
The smallest bit-string is produced by both Apache Avro \cite{avro} and
Protocol Buffers \cite{protocolbuffers} (0 bytes), closely followed by both
ASN.1 PER Unaligned \cite{asn1-per} and Apache Thrift \cite{slee2007thrift} (1
byte), and Cap'n Proto Packed Encoding \cite{capnproto} (7 bytes). Apache Avro
and Protocol Buffers achieve a zero byte-size as the input document consists of
a set of \emph{null} values, which these serialization specifications represent by not
encoding the corresponding fields.  The binary serialization specifications that
produced the smallest bit-strings are schema-driven, and with the exception of
Cap'n Proto Packed Encoding, which takes the fifth place, they are also
sequential. Conversely, the largest bit-string is produced by FlexBuffers
\cite{flexbuffers} (37 bytes), followed by Smile \cite{smile} (30 bytes) and
both BSON \cite{bson} and UBJSON \cite{ubjson} (29 bytes). The binary
serialization specifications that produced the largest bit-strings are schema-less and
with the exception of FlexBuffers, they are also sequential \cite{viotti2022survey}.  In
comparison to JSON \cite{ECMA-404} (44 bytes), binary serialization achieves 0
bytes in the best case for this input document, the maximal possible size
reduction. Additionally, none of the 14 JSON-compatible binary serialization
specifications listed in \autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON.

For this Tier 1 BRF document, the best performing schema-less serialization
specifications are CBOR \cite{RFC7049} and MessagePack \cite{messagepack} (25 bytes).
As shown in \autoref{table:benchmark-stats-sapcloudsdkpipeline}, uncompressed
schema-driven specifications provide smaller \emph{average} and \emph{median}
bit-strings than uncompressed schema-less specifications. However, as highlighted by
the \emph{range} and \emph{standard deviation}, uncompressed schema-driven
specifications exhibit higher size reduction variability depending on the
expressiveness of the schema language (i.e. how the language constructs allow
you to model the data) and the size optimizations devised by its authors.  The
entire selection of schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing
pointer-based serialization specification is Cap'n Proto Packed Encoding
\cite{capnproto} (7 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} do not result in positive
gains for any bit-string. The best performing compression format for JSON is
GZIP \cite{RFC1952} (50 bytes).


==> discussions/travisnotifications.tex <==
In this exceptional case, the smallest bit-string for this input document is
produced by the schema-less pointer-based serialization specification FlexBuffers
\cite{flexbuffers} (228 bytes), followed by the schema-driven sequential
specifications ASN.1 PER Unaligned \cite{asn1-per} (497 bytes) and Apache Avro
\cite{avro} (504 bytes). In comparison to other specifications, FlexBuffers detects
and de-duplicates the 7 instances of the same string value from this input
document. Conversely, the largest bit-string is produced by BSON \cite{bson}
(699 bytes), followed by FlatBuffers \cite{flatbuffers} (668 bytes) and UBJSON
\cite{ubjson} (658 bytes). With the exception of FlatBuffers, the binary
serialization specifications that produced the largest bit-strings are schema-less and
sequential \cite{viotti2022survey}.  In comparison to JSON \cite{ECMA-404} (673 bytes), binary
serialization achieves a \textbf{2.9x} size reduction in the best case for this
input document.  However, 1 out of the 14 JSON-compatible binary serialization
specifications listed in \autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: the schema-less and sequential BSON \cite{bson} binary
serialization specification.

For this Tier 2 TRF document, the smaller bit-string is produced by a
schema-less specification. The best performing schema-less serialization specification
achieves a \textbf{2.1x} size reduction compared to the best performing
schema-driven serialization specification: ASN.1 PER Unaligned \cite{asn1-per} (497
bytes).  As shown in \autoref{table:benchmark-stats-travisnotifications},
uncompressed schema-driven specifications provide smaller \emph{average} and
\emph{median} bit-strings than uncompressed schema-less specifications. Additionally,
as highlighted by the \emph{range} and \emph{standard deviation}, uncompressed
schema-less specifications exhibit higher size reduction variability given that
FlexBuffers \cite{flexbuffers} produces a notably small bit-string.  The
schema-less and pointer-based specification FlexBuffers \cite{flexbuffers} produces
bit-strings that are smaller to all their schema-driven counterparts listed in
\autoref{table:benchmark-specifications-schema-driven}.  The best performing
pointer-based serialization specification achieves a \textbf{2.1x} size reduction
compared to the best performing sequential serialization specification: ASN.1 PER
Unaligned \cite{asn1-per} (497 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
all bit-strings. The best performing compression format for JSON, GZIP
\cite{RFC1952} (154 bytes), achieves a \textbf{1.4x} size reduction compared to
the best performing uncompressed binary serialization specification.


==> discussions/tslintbasic.tex <==
The smallest bit-string is produced by both ASN.1 PER Unaligned \cite{asn1-per}
and Apache Avro \cite{avro} (1 byte), followed by both Protocol Buffers
\cite{protocolbuffers} and Apache Thrift \cite{slee2007thrift} (8 bytes), and
Microsoft Bond \cite{microsoft-bond} (9 bytes). The binary serialization
specifications that produced the smallest bit-strings are schema-driven and sequential
\cite{viotti2022survey}. Conversely, the largest bit-string is produced by FlexBuffers
\cite{flexbuffers} (77 bytes), closely followed by BSON \cite{bson} (71 bytes)
and FlatBuffers \cite{flatbuffers} (60 bytes). With the exception of BSON, the
binary serialization specifications that produced the largest bit-strings are
pointer-based \cite{viotti2022survey}.  In comparison to JSON \cite{ECMA-404} (67 bytes),
binary serialization achieves a \textbf{67x} size reduction in the best case
for this input document. Similar large size reductions are observed in JSON
documents whose content is dominated by \emph{boolean} and \emph{numeric}
values.  However, 2 out of the 14 JSON-compatible binary serialization specifications
listed in \autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: BSON \cite{bson} and FlexBuffers \cite{flexbuffers}.  These
binary serialization specifications are schema-less.

For this Tier 1 BNN document, the best performing schema-driven serialization
specification achieves a \textbf{51x} size reduction compared to the best performing
schema-less serialization specification: MessagePack \cite{messagepack} (51 bytes).
As shown in \autoref{table:benchmark-stats-tslintbasic}, uncompressed
schema-driven specifications provide smaller \emph{average} and \emph{median}
bit-strings than uncompressed schema-less specifications. However, as highlighted by
the \emph{range} and \emph{standard deviation}, uncompressed schema-driven
specifications exhibit higher size reduction variability depending on the
expressiveness of the schema language (i.e. how the language constructs allow
you to model the data) and the size optimizations devised by its authors.  With
the exception of the pointer-based binary serialization specification FlatBuffers
\cite{flatbuffers}, the selection of schema-driven serialization specifications listed
in \autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification achieves a \textbf{12x} size reduction compared to the
best performing pointer-based serialization specification: Cap'n Proto Packed Encoding
\cite{capnproto} (12 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
the bit-strings produced by Cap'n Proto Binary Encoding \cite{capnproto},
FlatBuffers \cite{flatbuffers} and FlexBuffers \cite{flexbuffers}. The best
performing uncompressed binary serialization specification achieves a
\textbf{68x} size reduction compared to the best performing compression format
for JSON: GZIP \cite{RFC1952} (68 bytes).


==> discussions/tslintextend.tex <==
The smallest bit-string is produced by ASN.1 PER Unaligned \cite{asn1-per} (46
bytes), closely followed by both Apache Avro \cite{avro} and Protocol Buffers
\cite{protocolbuffers} (47 bytes), and Apache Thrift \cite{slee2007thrift} (48
bytes). The binary serialization specifications that produced the smallest bit-strings
are schema-driven and sequential \cite{viotti2022survey}.  Conversely, the largest bit-string
is produced by both Cap'n Proto Binary Encoding \cite{capnproto} and
FlatBuffers \cite{flatbuffers} (88 bytes), followed by BSON \cite{bson} (78
bytes) and FlexBuffers \cite{flexbuffers} (70 bytes). With the exception of
BSON, the binary serialization specifications that produced the largest bit-strings
are pointer-based \cite{viotti2022survey}.  In comparison to JSON \cite{ECMA-404} (63 bytes),
binary serialization only achieves a \textbf{1.3x} size reduction in the best
case for this input document.  Additionally, 4 out of the 14 JSON-compatible
binary serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: Cap'n Proto Binary Encoding \cite{capnproto}, FlatBuffers
\cite{flatbuffers}, BSON \cite{bson} and FlexBuffers \cite{flexbuffers}. These
binary serialization specifications are either schema-less or schema-driven and
pointer-based.

For this Tier 1 TNF document, the best performing schema-driven serialization
specification only achieves a \textbf{1.1x} size reduction compared to the best
performing schema-less serialization specification: CBOR \cite{RFC7049} and
MessagePack \cite{messagepack} (55 bytes).  As shown in
\autoref{table:benchmark-stats-tslintextend}, uncompressed schema-driven
specifications provide smaller \emph{average} and \emph{median} bit-strings than
uncompressed schema-less specifications. However, as highlighted by the \emph{range}
and \emph{standard deviation}, uncompressed schema-driven specifications exhibit
higher size reduction variability depending on the expressiveness of the schema
language (i.e. how the language constructs allow you to model the data) and the
size optimizations devised by its authors.  With the exception of the
pointer-based binary serialization specifications Cap'n Proto Binary Encoding
\cite{capnproto}, Cap'n Proto Packed Encoding \cite{capnproto} and FlatBuffers
\cite{flatbuffers}, the selection of schema-driven serialization specifications listed
in \autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification only achieves a \textbf{1.3x} size reduction compared to
the best performing pointer-based serialization specification: Cap'n Proto Packed
Encoding \cite{capnproto} (62 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
the bit-strings produced by Cap'n Proto Binary Encoding \cite{capnproto} and
FlatBuffers \cite{flatbuffers}. The best performing uncompressed binary
serialization specification achieves a \textbf{1.5x} size reduction compared to
the best performing compression format for JSON: GZIP \cite{RFC1952} (70
bytes).


==> discussions/tslintmulti.tex <==
The smallest bit-string is produced by ASN.1 PER Unaligned \cite{asn1-per} (4
bytes), followed by Apache Avro \cite{avro} (7 bytes) and both Protocol Buffers
\cite{protocolbuffers} and Apache Thrift \cite{slee2007thrift} (14 bytes). The
binary serialization specifications that produced the smallest bit-strings are
schema-driven and sequential \cite{viotti2022survey}.  Conversely, the largest bit-string is
produced by BSON \cite{bson} (104 bytes), closely followed by FlexBuffers
\cite{flexbuffers} (102 bytes) and FlatBuffers \cite{flatbuffers} (84 bytes).
With the exception of BSON, the binary serialization specifications that produced the
largest bit-strings are pointer-based \cite{viotti2022survey}.  In comparison to JSON
\cite{ECMA-404} (98 bytes), binary serialization achieves a \textbf{24.5x} size
reduction in the best case for this input document. Similar large size
reductions are observed in JSON documents whose content is dominated by
\emph{boolean} and \emph{numeric} values. However, 2 out of the 14
JSON-compatible binary serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} and
\autoref{table:benchmark-specifications-schema-less} result in bit-strings that are
larger than JSON: BSON \cite{bson} and FlexBuffers \cite{flexbuffers}. These
binary serialization specifications are schema-less.

For this Tier 1 BRN document, the best performing schema-driven serialization
specification achieves a \textbf{17x} size reduction compared to the best performing
schema-less serialization specification: CBOR \cite{RFC7049} and MessagePack
\cite{messagepack} (68 bytes).  As shown in
\autoref{table:benchmark-stats-tslintmulti}, uncompressed schema-driven specifications
provide smaller \emph{average} and \emph{median} bit-strings than uncompressed
schema-less specifications. However, as highlighted by the \emph{range} and
\emph{standard deviation}, uncompressed schema-driven specifications exhibit higher
size reduction variability depending on the expressiveness of the schema
language (i.e. how the language constructs allow you to model the data) and the
size optimizations devised by its authors.  With the exception of the
pointer-based binary serialization specifications Cap'n Proto Binary Encoding
\cite{capnproto} and FlatBuffers \cite{flatbuffers}, the selection of
schema-driven serialization specifications listed in
\autoref{table:benchmark-specifications-schema-driven} produce bit-strings that are
equal to or smaller than their schema-less counterparts listed in
\autoref{table:benchmark-specifications-schema-less}.  The best performing sequential
serialization specification achieves a \textbf{5.7x} size reduction compared to the
best performing pointer-based serialization specification: Cap'n Proto Packed Encoding
\cite{capnproto} (23 bytes).

The compression formats listed in
\autoref{sec:benchmark-compression-formats} result in positive gains for
the bit-strings produced by Cap'n Proto Binary Encoding \cite{capnproto},
FlatBuffers \cite{flatbuffers}, JSON \cite{ECMA-404} and BSON \cite{bson}. The
best performing uncompressed binary serialization specification achieves a
\textbf{22.5x} size reduction compared to the best performing compression
format for JSON: GZIP \cite{RFC1952} (90 bytes).


==> introductions/circleciblank.tex <==
CircleCI \footnote{\url{https://circleci.com}} is a commercial cloud-provider
of continuous integration and deployment pipelines used by a wide range of
companies in the software development industry such as Facebook, Spotify, and
Heroku \footnote{\url{https://circleci.com/customers/}}. In
\autoref{fig:benchmark-circleciblank}, \we demonstrate a \textbf{Tier 1
minified $<$ 100 bytes numeric non-redundant flat} (Tier 1 NNF from
\autoref{table:json-taxonomy}) JSON document that represents a simple pipeline
configuration file for CircleCI that declares the desired CircleCI version
without defining any workflows.


==> introductions/circlecimatrix.tex <==
CircleCI \footnote{\url{https://circleci.com}} is a commercial cloud-provider
of continuous integration and deployment pipelines used by a wide range of
companies in the software development industry such as Facebook, Spotify, and
Heroku \footnote{\url{https://circleci.com/customers/}}. In
\autoref{fig:benchmark-circlecimatrix}, \we demonstrate a \textbf{Tier 1
minified $<$ 100 bytes numeric non-redundant nested} (Tier 1 NNN from
\autoref{table:json-taxonomy}) JSON document that represents a pipeline
configuration file for CircleCI that declares the desired CircleCI version and
defines a workflow that contains a single blank matrix-based job.


==> introductions/commitlint.tex <==
CommitLint \footnote{\url{https://commitlint.js.org/\#/}} is an open-source
command-line tool to enforce version-control commit conventions in software
engineering projects. CommitLint is a community effort under the Conventional
Changelog \footnote{\url{https://github.com/conventional-changelog}}
organization formed by employees from companies including GitHub
\footnote{\url{https://github.com/zeke}} and Google
\footnote{\url{https://github.com/bcoe}}. In
\autoref{fig:benchmark-commitlint}, \we demonstrate a \textbf{Tier 1 minified
$<$ 100 bytes textual redundant nested} (Tier 1 TRN from
\autoref{table:json-taxonomy}) JSON document that represents a CommitLint
configuration file which declares that the subject and the scope of any commit
must be written in lower-case form.


==> introductions/commitlintbasic.tex <==
CommitLint \footnote{\url{https://commitlint.js.org/\#/}} is an open-source
command-line tool to enforce version-control commit conventions in software
engineering projects. CommitLint is a community effort under the Conventional
Changelog \footnote{\url{https://github.com/conventional-changelog}}
organization formed by employees from companies including GitHub
\footnote{\url{https://github.com/zeke}} and Google
\footnote{\url{https://github.com/bcoe}}. In
\autoref{fig:benchmark-commitlintbasic}, \we demonstrate a \textbf{Tier 1
minified $<$ 100 bytes boolean non-redundant flat} (Tier 1 BNF from
\autoref{table:json-taxonomy}) JSON document that represents a CommitLint
configuration file which declares that CommitLint must not use its default
commit ignore rules.


==> introductions/epr.tex <==
Entry Point Regulation (EPR) \cite{EPR} is a W3C proposal led by Google that
defines a manifest that protects websites against cross-site scripting attacks
by allowing the developer to mark the areas of the application that can be
externally referenced. EPR manifests are used in the web industry. In
\autoref{fig:benchmark-epr}, \we demonstrate a \textbf{Tier 2 minified $\geq$
100 $<$ 1000 bytes textual redundant nested} (Tier 2 TRN from
\autoref{table:json-taxonomy}) JSON document that defines an example EPR policy
for a fictitious website.


==> introductions/eslintrc.tex <==
ESLint \footnote{\url{https://eslint.org}} is a popular open-source extensible
linter for the JavaScript \cite{ECMA-262} programming language used by a wide
range of companies in the software development industry such as Google,
Salesforce, and Airbnb. In \autoref{fig:benchmark-eslintrc}, \we demonstrate a
\textbf{Tier 3 minified $\geq$ 1000 bytes numeric redundant flat} (Tier 3 NRF
from \autoref{table:json-taxonomy}) JSON document that defines a browser and
Node.js linter configuration that defines general-purposes and
\emph{React.js}-specific \footnote{\url{https://reactjs.org}} linting rules.


==> introductions/esmrc.tex <==
\texttt{esm} \footnote{\url{https://github.com/standard-things/esm}} is an
open-source ECMAScript \cite{ECMA-262} module loader for the Node.js
\footnote{\url{https://nodejs.org}} JavaScript runtime that allows developers
to use the modern \texttt{import} module syntax on older runtime versions.
\texttt{esm} is used in the web industry. In \autoref{fig:benchmark-esmrc}, \we
demonstrate a \textbf{Tier 2 minified $\geq$ 100 $<$ 1000 bytes boolean
non-redundant flat} (Tier 2 BNF from \autoref{table:json-taxonomy}) JSON
document that defines an example \texttt{esm} configuration.


==> introductions/geojson.tex <==
GeoJSON \cite{RFC7946} is a standard to encode geospatial information using
JSON. GeoJSON is used in industries that have geographical and geospatial use
cases such as engineering, logistics and telecommunications. In
\autoref{fig:benchmark-geojson}, \we demonstrate a \textbf{Tier 2 minified
$\geq$ 100 $<$ 1000 bytes numeric redundant nested} (Tier 2 NRN from
\autoref{table:json-taxonomy}) JSON document that defines an example polygon
using the GeoJSON format.


==> introductions/githubfundingblank.tex <==
The GitHub \footnote{\url{https://github.com}} software hosting provider
defines a \texttt{FUNDING}
\footnote{\url{https://docs.github.com/en/github/administering-a-repository/managing-repository-settings/displaying-a-sponsor-button-in-your-repository}}
file format to declare the funding platforms that an open-source project
supports. The \texttt{FUNDING} file format is used by the open-source software
industry. In \autoref{fig:benchmark-githubfundingblank}, \we demonstrate a
\textbf{Tier 2 minified $\geq$ 100 $<$ 1000 bytes boolean redundant flat} (Tier
2 BRF from \autoref{table:json-taxonomy}) JSON document that consists of a
definition that does not declare any supported funding platforms.


==> introductions/githubworkflow.tex <==
The GitHub \footnote{\url{https://github.com}} software hosting provider has an
automation service called GitHub Actions
\footnote{\url{https://github.com/features/actions}} for projects to define
custom workflows. GitHub Actions is used primarily by the open-source software
industry. In \autoref{fig:benchmark-githubworkflow}, \we demonstrate a
\textbf{Tier 2 minified $\geq$ 100 $<$ 1000 bytes textual non-redundant nested}
(Tier 2 TNN from \autoref{table:json-taxonomy}) JSON document that consists of
a simple example workflow definition.


==> introductions/gruntcontribclean.tex <==
Grunt.js \footnote{\url{https://gruntjs.com}} is an open-source task runner for
the JavaScript \cite{ECMA-262} programming language used by a wide range of
companies in the software development industry such as Twitter, Adobe, and
Mozilla \footnote{\url{https://gruntjs.com/who-uses-grunt}}. In
\autoref{fig:benchmark-gruntcontribclean}, \we demonstrate a \textbf{Tier 1
minified $<$ 100 bytes textual redundant flat} (Tier 1 TRF from
\autoref{table:json-taxonomy}) JSON document that consists of an example
configuration for a built-in plugin to clear files and folders called
\texttt{grunt-contrib-clean}
\footnote{\url{https://github.com/gruntjs/grunt-contrib-clean}}.


==> introductions/imageoptimizerwebjob.tex <==
Image Optimizer
\footnote{\url{https://github.com/madskristensen/ImageOptimizerWebJob}} is an
Azure App Services WebJob
\footnote{\url{https://docs.microsoft.com/en-us/azure/app-service/webjobs-create}}
to compress website images used in the web development industry. In
\autoref{fig:benchmark-imageoptimizerwebjob}, \we demonstrate a \textbf{Tier 1
minified $<$ 100 bytes textual non-redundant nested} (Tier 1 TNN from
\autoref{table:json-taxonomy}) JSON document that consists of an Image
Optimizer configuration to perform lossy compression on images inside a
particular folder.


==> introductions/jsonereversesort.tex <==
JSON-e \footnote{\url{https://github.com/taskcluster/json-e}} is an open-source
JSON-based templating engine created by Mozilla as part of the TaskCluster
\footnote{\url{https://taskcluster.net}} project, the open-source task
execution framework that supports Mozilla's continuous integration and release
processes. In \autoref{fig:benchmark-jsonereversesort}, \we demonstrate a
\textbf{Tier 1 minified $<$ 100 bytes numeric redundant nested} (Tier 1 NRN
from \autoref{table:json-taxonomy}) JSON document that consists of an example
JSON-e template definition to sort and reverse an array of numbers.


==> introductions/jsonesort.tex <==
JSON-e \footnote{\url{https://github.com/taskcluster/json-e}} is an open-source
JSON-based templating engine created by Mozilla as part of the TaskCluster
\footnote{\url{https://taskcluster.net}} project, the open-source task
execution framework that supports Mozilla's continuous integration and release
processes. In \autoref{fig:benchmark-jsonesort}, \we demonstrate a \textbf{Tier
1 minified $<$ 100 bytes numeric redundant flat} (Tier 1 NRF from
\autoref{table:json-taxonomy}) JSON document that consists of an example JSON-e
template definition to sort an array of numbers.


==> introductions/jsonfeed.tex <==
JSON Feed \cite{jsonfeed} is a specification for a syndication JSON format
similar to RSS \cite{rss} and Atom \cite{RFC4287} used in the publishing
\footnote{\url{https://micro.blog}} and media
\footnote{\url{https://npr.codes/npr-now-supports-json-feed-1c8af29d0ce7}}
industries. In \autoref{fig:benchmark-jsonfeed}, \we demonstrate a \textbf{Tier
2 minified $\geq$ 100 $<$ 1000 bytes textual non-redundant flat} (Tier 2 TNF
from \autoref{table:json-taxonomy}) JSON document that consists of a JSON Feed
manifest for an example website that contains a single blog entry.


==> introductions/jsonresume.tex <==
JSON Resume \footnote{\url{https://jsonresume.org}} is a community-driven
proposal for a JSON-based file format that declares and renders themable
resumes used in the recruitment industry. In
\autoref{fig:benchmark-jsonresume}, \we demonstrate a \textbf{Tier 3 minified
$\geq$ 1000 bytes textual non-redundant nested} (Tier 3 TNN from
\autoref{table:json-taxonomy}) JSON document that consists of a detailed
example resume for a fictitious software programmer.


==> introductions/netcoreproject.tex <==
The ASP.NET \footnote{\url{https://dotnet.microsoft.com/apps/aspnet}} Microsoft
web-application framework defined a now-obsolete JSON-based project manifest
called \texttt{project.json}
\footnote{\url{http://web.archive.org/web/20150322033428/https://github.com/aspnet/Home/wiki/Project.json-file}}
used in the web industry. In \autoref{fig:benchmark-netcoreproject}, \we
demonstrate a \textbf{Tier 3 minified $\geq$ 1000 bytes textual redundant
nested} (Tier 3 TRN from \autoref{table:json-taxonomy}) JSON document that
consists of a detailed an example \texttt{project.json} manifest that lists
several dependencies.


==> introductions/nightwatch.tex <==
Nightwatch.js \footnote{\url{https://nightwatchjs.org}} is an open-source
browser automation solution used in the software testing industry. In
\autoref{fig:benchmark-nightwatch}, \we demonstrate a \textbf{Tier 3 minified
$\geq$ 1000 bytes boolean redundant flat} (Tier 3 BRF from
\autoref{table:json-taxonomy}) JSON document that consists of a Nightwatch.js
configuration file that defines a set of general-purpose WebDriver
\cite{webdriver} and Selenium \footnote{\url{https://www.selenium.dev}}
options.


==> introductions/openweathermap.tex <==
OpenWeatherMap \footnote{\url{https://openweathermap.org}} is a weather data
and forecast API provider used in industries such as energy, agriculture,
transportation and construction. In \autoref{fig:benchmark-openweathermap}, \we
demonstrate a \textbf{Tier 2 minified $\geq$ 100 $<$ 1000 bytes numeric
non-redundant flat} (Tier 2 NNF from \autoref{table:json-taxonomy}) JSON
document that consists of an HTTP/1.1 \cite{RFC7231} response of the weather
information in Mountain View, California on June 12, 2019 at 2:44:05 PM GMT.


==> introductions/openweatherroadrisk.tex <==
OpenWeatherMap \footnote{\url{https://openweathermap.org}} is a weather data
and forecast API provider used in industries such as energy, agriculture,
transportation and construction. In
\autoref{fig:benchmark-openweatherroadrisk}, \we demonstrate a \textbf{Tier 2
minified $\geq$ 100 $<$ 1000 bytes numeric non-redundant nested} (Tier 2 NNN
from \autoref{table:json-taxonomy}) JSON document that consists of an example
HTTP/1.1 \cite{RFC7231} Road Risk API response from the official API
documentation that provides weather data and national alerts along a specific
route.


==> introductions/packagejson.tex <==
Node.js Package Manager (NPM) \footnote{\url{https://www.npmjs.com}} is an
open-source package manager for Node.js \footnote{\url{https://nodejs.org}}, a
JavaScript \cite{ECMA-262} runtime targetted at the web development industry. A
package that is published to NPM is declared using a JSON file called
\texttt{package.json}
\footnote{\url{https://docs.npmjs.com/cli/v6/configuring-npm/package-json}}.
In \autoref{fig:benchmark-packagejson}, \we demonstrate a \textbf{Tier 3
minified $\geq$ 1000 bytes textual non-redundant flat} (Tier 3 TNF from
\autoref{table:json-taxonomy}) JSON document that consists of a
\texttt{package.json} manifest that declares a particular version of the
Grunt.js \footnote{\url{https://gruntjs.com}} task runner.


==> introductions/packagejsonlintrc.tex <==
Node.js Package Manager (NPM) \footnote{\url{https://www.npmjs.com}} is an
open-source package manager for Node.js \footnote{\url{https://nodejs.org}}, a
JavaScript \cite{ECMA-262} runtime targetted at the web development industry.
\texttt{npm-package-json-lint}
\footnote{\url{https://npmpackagejsonlint.org/en/}} is an open-source tool to
enforce a set of configurable rules for a Node.js Package Manager (NPM)
\footnote{\url{https://www.npmjs.com}} configuration manifest. In
\autoref{fig:benchmark-packagejsonlintrc}, \we demonstrate a \textbf{Tier 3
minified $\geq$ 1000 bytes textual redundant flat} (Tier 3 TRF from
\autoref{table:json-taxonomy}) JSON document that consists of an example
\texttt{npm-package-json-lint} configuration.


==> introductions/sapcloudsdkpipeline.tex <==
SAP Cloud SDK \footnote{\url{https://sap.github.io/cloud-sdk/}} is a framework
that includes support for continuous integration and delivery pipelines to
develop applications for the SAP
\footnote{\url{https://www.sap.com/index.html}} enterprise resource planning
platform used by industries such as finance, healthcare and retail. In
\autoref{fig:benchmark-sapcloudsdkpipeline}, \we demonstrate a \textbf{Tier 1
minified $<$ 100 bytes boolean redundant flat} (Tier 1 BRF from
\autoref{table:json-taxonomy}) JSON document that defines a blank pipeline with
no declared steps.


==> introductions/travisnotifications.tex <==
TravisCI \footnote{\url{https://travis-ci.com}} is a commercial cloud-provider
of continuous integration and deployment pipelines  used by a wide range of
companies in the software development industry such as ZenDesk, BitTorrent, and
Engine Yard. In \autoref{fig:benchmark-travisnotifications}, \we demonstrate a
\textbf{Tier 2 minified $\geq$ 100 $<$ 1000 bytes textual redundant flat} (Tier
2 TRF from \autoref{table:json-taxonomy}) JSON document that consists of an
example pipeline configuration for TravisCI that declares a set of credentials
to post build notifications to various external services.


==> introductions/tslintbasic.tex <==
TSLint \footnote{\url{https://palantir.github.io/tslint}} is now an obsolete
open-source linter for the TypeScript
\footnote{\url{https://www.typescriptlang.org}} programming language. TSLint
was created by the Big Data analytics company Palantir
\footnote{\url{https://www.palantir.com}} and was merged with the ESLint
open-source JavaScript linter in 2019
\footnote{\url{https://github.com/palantir/tslint/issues/4534}}. In
\autoref{fig:benchmark-tslintbasic}, \we demonstrate a \textbf{Tier 1 minified
$<$ 100 bytes boolean non-redundant nested} (Tier 1 BNN from
\autoref{table:json-taxonomy}) JSON document that consists of a basic TSLint
configuration that enforces grouped alphabetized imports.


==> introductions/tslintextend.tex <==
TSLint \footnote{\url{https://palantir.github.io/tslint}} is now an obsolete
open-source linter for the TypeScript
\footnote{\url{https://www.typescriptlang.org}} programming language. TSLint
was created by the Big Data analytics company Palantir
\footnote{\url{https://www.palantir.com}} and was merged with the ESLint
open-source JavaScript linter in 2019
\footnote{\url{https://github.com/palantir/tslint/issues/4534}}. In
\autoref{fig:benchmark-tslintextend}, \we demonstrate a \textbf{Tier 1 minified
$<$ 100 bytes textual non-redundant flat} (Tier 1 TNF from
\autoref{table:json-taxonomy}) JSON document that consists of a basic TSLint
configuration that only extends a set of existing TSLint configurations.


==> introductions/tslintmulti.tex <==
TSLint \footnote{\url{https://palantir.github.io/tslint}} is now an obsolete
open-source linter for the TypeScript
\footnote{\url{https://www.typescriptlang.org}} programming language. TSLint
was created by the Big Data analytics company Palantir
\footnote{\url{https://www.palantir.com}} and was merged with the ESLint
open-source JavaScript linter in 2019
\footnote{\url{https://github.com/palantir/tslint/issues/4534}}. In
\autoref{fig:benchmark-tslintmulti}, \we demonstrate a \textbf{Tier 1 minified
$<$ 100 bytes boolean redundant nested} (Tier 1 BRN from
\autoref{table:json-taxonomy}) JSON document that consists of a TSLint
configuration that enables and configures a set of built-in rules.

